Applied Metamodelling: A Foundation for Language Driven Development (Third Edition)

Modern day system developers have some serious problems to contend with. The systems they develop are becoming increasingly complex as customers demand richer functionality delivered in ever shorter timescales. They have to manage a huge diversity of implementation technologies, design techniques and development processes: everything from scripting languages to web-services to the latest 'silver bullet' design abstraction. To add to that, nothing stays still: today's 'must have' technology rapidly becomes tomorrow's legacy problem that must be managed along with everything else. How can these problems be dealt with? In this book we propose that there is a common foundation to their resolution: languages. Languages are the primary way in which system developers communicate, design and implement systems. Languages provide abstractions that can encapsulate complexity, embrace the diversity of technologies and design abstractions, and unite modern and legacy systems.

==> AbstractSyntax/staticOO.tex <==
\section{Case Study 2: A simple OO modelling language}

This section presents a metamodel of a simple OO modelling language, which we call OML. OML is essentially a cut down version of UML and MOF. Whilst metamodels already exists for UML and MOF, they are complex, due to the rich set of modelling concepts they provide. Therefore, the metamodel presented here focuses on the most basic primitives necessary to express OO models.

As an example, figure \ref{omlexample} shows a simple model written in the language of OML.
The details of the model, a simple Bank in this case, are not particularly important. What is important is that it provides an example of the modelling concepts that are used by OML. These include the following:

\begin{figure}[htb]
\begin{center}
\includegraphics[width=13cm]{MetamodellingLanguages/StaticStructure/figures/OMLexample.pdf}
\caption{A simple OML model}
\label{omlexample}
\end{center}
\end{figure}

\begin{description}
\item [Class] A class is an abstraction of a collection of objects. A class has a name, and a set of attributes. A class may be related to another class by generalisation, in which case the more specific class is viewed as inheriting the properties of the more general class.
\item [Package] A package is a container of modelling elements, including classes. A package may contain other packages.
\item [Attribute] An attribute describes a particular property of a class. Attributes have a name and a type. A type may be a simple type, e.g. an Integer or a String, or a complex type, such as a class, or a collection of classes.
\end{description}

As explained in section, a useful exercise when identifying concepts in a language, is to annotate example models with the modelling concepts that they can be viewed as being instances of. Figure \ref{omlannotatedexample} shows the Bank example annotated with the modelling concepts that are in OML.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=13cm]{MetamodellingLanguages/StaticStructure/figures/OMLannotatedexample.pdf}
\caption{An annotated OML model}
\label{omlannotatedexample}
\end{center}
\end{figure}

The representation of an attribute with a simple type versus an attribute with complex type is worth noting here. Whilst the concept is the same, the representation (concrete syntax) is quite different: a textual representation versus a diagrammatical one. In fact, there is nothing to prevent there being two or more ways of representing exactly the same concept. A textual representation of an attribute with a complex type could also have been used, e.g. accounts : Set{Account}.
As will be discussed in chapter{concretesyntax}, a concrete syntax merely provides (possibly multiple) views on the concepts in an abstract syntax metamodel.

\subsection{Metamodel}

Figure ? shows the result of translating the identified concepts into an abstractsyntax metamodel.

==> AbstractSyntax/static_with_DFDs.tex <==
\chapter{Abstract Syntax Metamodels}
\label{abschapter}

\section{Introduction}

Just as a the quintessential step in object oriented design is constructing a model of system concepts, constructing an abstract syntax metamodel is an essential first step in the design of a modelling language. An abstract syntax metamodel describes the concepts in the language and their relationships to each other. In addition, it also defines the rules that determine whether a model written in the language is valid or not. These are the well-formedness rules of the language. 

Imagine a business modelling language suitable for modelling high level business rules about business data. An appropriate language for this domain might provide modelling concepts such as "data model", "data entity", and "business rule". In addition, there will be relationships between these concepts: a "data model" may be composed of a number of "data entities". There will also be rules describing the valid models that may be constructed in the language, for instance, "a datamodel cannot contain two or more data entities with the same name" might be one such rule. 

The concepts, relationships and rules identified during this step will provide a vocabulary and grammar for constructing models in the language. This will act as a foundation upon which all other artefacts of the language design process will be rooted.  

This chapter describes the steps required to construct abstract syntax metamodels, along with examples of their application to the definition of the abstract syntax model of a simple modelling language. 

\section{Modelling Abstract Syntax}

As stated, the purpose of an abstract syntax metamodel is to describe the concepts in a language and the relationships that exist between those concepts. In the context of a language definition, a concept is anything that represents a part of the vocabulary of the language. The term abstract syntax emphasises a focus on the the abstract representation of the concepts, as opposed to the notation of the concepts or their semantics. As a result, abstract syntax metamodels tend to focus on the static, syntactical properties of concepts in a language. Note that it is not the purpose of the abstract syntax metamodel to describe the semantics of the language, or how it will be presented. These aspects will be described later.

In addition, an abstract syntax metamodel should also describe the rules by which a model written in the language is deemed to be well-formed, i.e. is syntactically valid. These provide a more detailed description of the syntactical rules of the language than is possible just by describing the concepts and relationships alone. These well-formedness rules are particularly useful when it comes to implementing a tool to support the language, as they can be used to validate the correctness of models as they are created.

Constructing an abstract syntax metamodel has much in common with developing an abstract grammar for a programming language, albeit that the language used is more expressive than that used in programming language design. 

Abstract syntax metamodels are written in a metamodelling language. As described in chapter \ref{xmofchapter}, the metamodelling language we will use, called XMOF, provides a number of modelling abstractions suitable for modelling languages. For the purposes of modelling abstract syntax, only a subset of XMOF will be required. This is the subset suitable for capturing the static properties of language concepts and rules of well-formedness, and includes:

\begin{itemize}
\item classes to describe the concepts in the language;
\item packages to partition the metamodel into manageable chunks where necessary.
\item attributes and associations to describe the relationships between concepts;
\item constraints, written in OCL, to express the well-formedness rules.
\end{itemize} 

\section{The Process}

There are a number of stages involved in developing an abstract syntax metamodel: concept identification; concept modelling; model architecting; model validation and model testing. These stages are described below.

\subsection{Concept Identification}
\label{conceptidentification}

The first stage in modelling the abstract syntax of a language is to utilise any information available to help in identifying the concepts that the language uses, and any obvious rules regarding valid and invalid models. 

There are a number of useful techniques that can be used to help in this process:

\begin{itemize}

\item Construct a list of candidate concepts in the language. Focus on determining whether the concepts make sense as part of the language's vocabulary. In particular, identify concepts that match the following criteria:

\begin{itemize}
  \item Concepts that have names.
   \item Concepts that contain other concepts, e.g. a class containing attributes.
  \item Concepts that record information about relationships with other concepts, e.g. named associations between classes.
  \item Concepts that play the role of namespaces for named concepts.
  \item Concepts that exhibit a type/instance relationship.
  \item Concepts that are recursively decomposed.
  \item Concepts that are a part of an expression, or which are associated with expressions.
\end{itemize}

\item Build examples of models using the language. 

\begin{itemize}
\item Utilise any notation that you think appropriate to represent each type of concept. Use this notation to build models of meaningful/real world examples. 
\item In the case of a pre-existing language there should be examples already available to help in the identification of concepts. Other good sources of inspiration include CASE tools, which will provide automated support for building example models. Such tools may also provide additional facilities for checking valid and invalid models, which will be useful when identifying well-formedness rules or may provide more detailed examples of the language syntax. 
\end{itemize}
 
\end{itemize}

Once some examples have been constructed, abstract away from them to identify the generic language concepts and relationships between concepts. It is often useful to annotate the examples with the modelling concepts as a precursor to this step. Examples of invalid models can also be used to help in the identification of well-formedness rules. 

It is important during this process to distinguish between the concrete syntax of a language and its abstract syntax. Whilst it is common for the structure of the abstract syntax to reflect its concrete syntax, this need not be the case. For example, consider a language which provides multiple, overlapping views of a small number of core modelling concepts. In this case, the abstract syntax should reflect the core modelling concepts, and not the concrete syntax. 

'Modelling the diagrams' is a common mistake made by many novice metamodellers. If in doubt, ask the following questions when identifying concepts:

\begin{itemize}
\item Does the concept have meaning, or is it there purely for presentation? If the latter, then it should be viewed as concrete syntax. An example might be a "Note", which clearly does not deserve to be modelled as an abstract syntax concept.
\item Is the concept a derived concept, or is it just a view on a collection of more primitive concepts? If so, a relationship should be defined between the richer concept and the more primitive concept. Consider a dataflow between a process and a datastore that is derived from the fact that the process has an action that updates the datastore. 
\end{itemize}

In general, the best abstract syntax models are the simplest ones. Any complexity due to diagrammatical representation should be deferred to the concrete syntax models.

\subsection{Concept Modelling}

Once concepts have been identified, standard OO modelling features, classes, packages, and associations are applied to model the concepts in the language. There are many examples of developing conceptual models available in the literature, for instance, \cite{Larman} devotes a significant amount of time to this subject. 

In general, concepts will be described using classes, with appropriate attributes used to capture the properties of the concepts. Some concepts will have relationships to other concepts, and these will be modelled as associations. Where it makes sense to define categories of concepts, generalization can be used to seperate them into more general and more specific types of concepts.

A useful strategy to apply at this stage is to reuse existing language definitions where possible. There are a number of techniques that can be used to achieve this, including:

\begin{itemize}
\item Extending or tailoring an existing metamodel to fit the new language. This can be achieved by specializing classes from the existing metamodel or by using package extension to import and extend whole packages of concepts.
\item Utilising language patterns. A language pattern may be realised as a framework of abstract classes that capture a repeatedly used language structure, or by a package template (a parameterized package).
\end{itemize}

\noindent A full discussion of these techniques will be presented in chapter ??.

\subsection{Well-formedness Rules and Operations}

Once a basic metamodel has been constructed, start identifying both legal and illegal examples of models that may be written in the language. Use this information to define a set of well-formedness rules in XOCL that rule out the illegal models. When defining rules, look to identify the most general rules possible, and investigate the implications of what happens when rules are combined - sometimes rules can conflict in unexpected ways. There are many books available on writing constraints in OCL that can help guide this process, see \cite{Warmer} for example. Reusing existing language components can also minimise the effort involved in writing well-formedness rules, as constraints can be reused as well - however, be aware that if specialisation is used then.

Operations and queries should also be defined where appropriate. Examples of operations include general utility operations such as creating new model elements and setting attribute values, or operations that act as test harnesses. Examples of queries might include querying properties of models for use in constraints and operations, or for validation purposes. Operations that change the state of models should take into account any constraints, ensuring that if a constraint holds before the operation is invoked, it will continue to hold afterwards.

\subsection{Use Cases}

A very useful technique to understanding and defining the properties of a modelling language is to consider the different use cases associated with using the language. This is almost akin to writing a metamodel API, i.e. a collection of operations that would be used when interacting with the metamodel. Some typical use cases might include creating and deleting model elements, but may also include semantically rich operations such as transforming a model, or executing a statemachine. Taken to its extremes, such an approach can be used to completely drive the identification of concepts in a metamodel: in effect a use case driven approach. However, as is always a case, an iterative process is always useful.

\subsection{Metamodel Integration}

At some point during the development of the abstract syntax model, it will need to be integrated within a specific metamodelling framework. This will enable it to take advantage of the generic mechanisms and APIs provided by the framework and will support its implementation in a tool. The XMOF framework provides generic mechanisms that includes model element instantiation, parsing and expression evaluation. Thus, an analysis of where the classes in the abstract syntax model need to extend or reference classes in the framework should be undertaken.

%More required here.

\subsection{Validation and Testing}

It is important to validate the correctness of the abstract syntax model. Investing in this early on will pay dividends in the longer run. A useful (static) technique for doing this is to construct instances of the abstract syntax metamodel that match those of example models. An object diagram is a useful way of capturing this information as it shows instances of classes (objects) and associations (links). There are tools available that will both help create object diagrams, and also check they are valid with respect to a model and any OCL constraints that have been defined. 

The best means of testing the correctness of a language definition is to build a tool that implements it. Only then, can the language be tested by end users in its entirety. Tools that facilitate the rapid generation of tools from metamodels are discussed in more detail in chapter ??.

\section{Case Study}

The best way to learn about metamodelling is to look at some real examples. An example of a simple, but widely known modelling language, is a data flow diagram, or DFD. DFD's were widely used in the 1980's and early 1990's as a notation for modelling the flow of data between entities in a system. Indeed they are still used today by data modellers as an important tool for eliciting data structures. DFD's are a good starting point for illustrating metamodelling as they are simple, but illustrated many facets of the metamodelling process.

As shown in figure \ref{dfdexample}, a DFD is essentially a visual network of data flows between processes, data stores and external entities, which aims to model the logical flow of data in a system and the transformations that occur to the data (without committing to physical implementation details). 

\begin{figure}[htb]
\begin{center}
\includegraphics[width=13cm]{AbstractSyntax/figures/DFDExample.pdf}
\caption{An example of a data flow diagram (DFD)}
\label{dfdexample}
\end{center}
\end{figure}

There are a number of other features of DFDs that are not illustrated by this example. One of the most important is the ability for processes to be nested. As shown in figure \ref{dfdnested} ,this enables a single process node on a high level diagram to be expanded to show a more detailed collections of processes. The highest level process in the DFD hierarchy is commonly called a context diagram. This provides a view of the system as a single process, along with the input and output dataflows that flow to and from the external entities to the system.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=13cm]{AbstractSyntax/figures/DFDContext.pdf}
\caption{A nested DFD}
\label{dfdnested}
\end{center}
\end{figure}

Processes can be decomposed to any level of detail. The diagram in figure \ref{addreader} shows the decomposition of the NewReader process.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=13cm]{AbstractSyntax/figures/AddReader.pdf}
\caption{Decomposing the NewReader process}
\label{addreader}
\end{center}
\end{figure}

Finally, in order to describe the effect of a leaf process, DFDs typically provide a simple action language. This can be a specification style language, such as Pspecs \cite{}, which describes the effect of the process in terms of pre- and post- conditions, or it can be an operational language. Because we ultimately wish to be able to execute the DFD's, the latter has been chosen. 

The action language supports a collection of simple actions for updating and reading records from datastores, making choices, and calling other actions in other processes.

\small
\begin{verbatim}
@Process AddReader(name)
  @When
    not Readers.records->exists(reader | reader->at(0) = name) 
  do
    @Block
      @Update Readers with Seq{name} end
      @OCLExp "ReaderAdded" end
    end
  end
end
\end{verbatim}
\normalsize    

The action illustrated here is a When action, which has a condition, that, if true, results in the activation of the action in the do expression. In this case, if no reader currently exists with the same name in the Readers datastore, a sequential Block action is called. This firstly updates the Readers datastore with a sequence containing the name of the reader and then produces the OCL string expression, "ReaderAdded".   

\subsection{Identification of Concepts}

Based on the example shown in figure \ref{dfdexample}, the following candidates for concepts can be immediately identified:

\begin{description}
\item [Process]  A transformer of information that resides within the bounds of the system to be modelled. Processes appear as named circles in a DFD.

\item [External Entity] A producer or consumer of information that resides outside the bounds of the system to be modelled. An external entity is drawn as a named box.

\item [Datastore] A repository of data records that is to be stored for use by one or more processes. A datastore is drawn as a half open box.

\item [Dataflow] Represents the flow of data between processes, entities and datastores. Dataflows are named and are uni-directional. Dataflows are shown as lines with a single arrow at one end, pointing in the direction of the flow.

\item [Action] An action belongs to a process and has a body which specifies the effect of the action. The following primitive sets of actions are provided: 
\begin{itemize}
\item A Send action causes a process in scope to be activated by sending the process a message.
\item An Update action is used to add a record to a data store.
\item A Remove action removes a record from a datastore.
\item An Or action performs a number of actions in sequence until one of them succeeds. 
\item A When action allows actions to be activated provided a condition holds.
\item A Block action contains a sequence of sub-actions, which are activated in order.
\item An OCLExp action that contains an XOCL expression which can be evaluated in the normal way.
\end{itemize}

\end{description}

Figure \ref{dfdannotated} shows the same DFD model 'marked up' with some of the identified concepts. A similar exercise can be carried out for elements in the action language example.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=13cm]{AbstractSyntax/figures/DFDAnnotated.pdf}
\caption{An annotated example of a data flow diagram (DFD)}
\label{dfdannotated}
\end{center}
\end{figure}

\subsection{The Model}

Once some candidate concepts have been identified, the next step is to construct the model. 

An important question to ask at this point is whether each concept is an appropriate abstract syntax concept. Datastores, processes and actions are clearly core to DFDs, as they capture the central concepts of data and data transformation. There is a question mark however over external entities and data flows:

\begin{itemize} 
\item External entities are external to the system being modelled, and would appear to be redundent in the sense that they only add contextual information. \item Dataflows appear to be derived concepts, as they could be thought of as showing information flow dependencies between processes and datastores as the result of actions. For instance, a flow from a process to a datastore can be derived from an action belonging to the process that updates the datastore.
\end{itemize}

\noindent For now, these two concepts will be put to one side \footnote{They will be considered further in the concrete syntax chapter}. 

By focusing on processes, datastores and actions, the model shown in figure \ref{dfdabs1} is obtained.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=10cm]{AbstractSyntax/figures/DFDAbs1.pdf}
\caption{An bstract syntax metamodel for DFDs}
\label{dfdabs1}
\end{center}
\end{figure}

There are a number of points to note about the model:

\begin{itemize}
\item Processes are associated with: the collection of datastores that are accessible by the process; a single action body; and the collection of sub-processes belonging to the process. A process has a single 'argument' that it uses to refer to input messages. The body of the process provides its output messages.
\item Datastores contain an attribute, fields, which defines the names of the elements in each of its records.
\item Any element that can be viewed as a component of a process is a specialisation of the class ProcessComponent. This provides an abstract operation, addTo(), which defines how a component adds itself to a process.
\item {\it When} expressions are associated with a collection of clauses, which define the rules for testing whether the body of the clause should be activated.
\end{itemize}

\subsection{Well-formedness Rules}

Whilst most of the concepts and relationship in the DFD language have been identified,  there are some important rules missing about what constitutes a well-formed DFD. Firstly, it must be the case that sub-processes and datastores associated with a process have unique names:

\small
\begin{verbatim}
context Process
@Constraint AllProcessesHaveUniqueNames
  processes->forAll(p1 |
    processes->forAll(p2 |
      p1.name = p2.name implies p1 = p2))
end

context Process
@Constraint AllDataStoresHaveUniqueNames
  dataStores->forAll(p1 |
    dataStores->forAll(p2 |
      p1.name = p2.name implies p1 = p2))
end
\end{verbatim}
\normalsize

Finally, there are some rules relating to nesting:

\begin{enumerate}
\item There should be no cyclic nesting of processes. This is required in order to avoid there being cyclic dependencies in a DFD.
\item Sub-processes must only have access to datastores that are accessible by their parent processes.
\end{enumerate}

\noindent These rules can be expressed as follows:

\small
\begin{verbatim}
context Process
@Constraint NoCyclicDependencies
  not self.allOwnedProcesses()->includes(self)
end  

context Process
@Constraint DatastoresAreInherited
   datastores->includesAll(processes.datastores)
\end{verbatim}
\normalsize

\noindent Where the definition of the operation allOwnedProcesses() is given by the following OCL expression:

\small
\begin{verbatim}
context Process
@Operation allOwnedProcesses():Set(Process)
  processes->
    collect(p | p.allOwnedProcess())
end  
\end{verbatim}
\normalsize

\subsection{Operations}

The following operations are defined for a process:

\small
\begin{verbatim}
context Process
@Operation addTo(p:Process)
  p.addProcess(self)
end

context Process
@Operation addStore(store:DataStore)
  self.dataStores := dataStores->including(store)
end

context Process
@Operation addProcess(process:Process)
  self.processes := processes->including(process)
end 
\end{verbatim}
\normalsize

The operation addTo() adds a process as a sub-process to the current process by calling the addProcess() operation. The addStore() operation adds a datastore to the collection of datastores that are accessible by the process.

The operation addTo() is similarly defined for a datastore:

\small
\begin{verbatim}
@Operation addTo(p:Process)
  p.addStore(self)
end
\end{verbatim}
\normalsize

As we shall see in chapter ??, these operations will become useful when populating DFDs during parsing.

\subsection{Validating the DFD metamodel}

In figure \ref{dfdsnapshot} a partial object diagram corresponding to the DFD in figure \ref{dfdexample} is shown. Here, instances of XOCL expressions are the values that are passed as expressions to the actions. The main point to note about this diagram is that it satisfies the well-formedness rules of the DFD. 

\begin{figure}[htb]
\begin{center}
\includegraphics[width=10cm]{AbstractSyntax/figures/DFDsnapshot.pdf}
\caption{An object diagram corresponding to figure \ref{dfdexample}}
\label{dfdsnapshot}
\end{center}
\end{figure}

However, this is about as far as we can go. At this point, the model is just a model of the abstract syntax and nothing more. To enable DFDs to be conveniently inputed, parsed and executed both the concrete syntax and semantics of the language must be modelled too. These aspects will be explored in the following chapters. 

\section{Conclusion}

This chapter has examined the process and modelling language required to model the abstract syntax of languages. The result is a definition of the concepts in a language and the relationship and rules that govern them. However, this is just a first step towards a complete definition of the language. Only once the concrete syntax and semantics of the language are modelled does it become a true metamodel.



==> CaseStudy1/DFD.tex <==
\chapter{Case Study 1: A Component Modelling Language}

\section{Introduction}

The best way to learn how to metamodel is to look at some real
examples. This chapter gives a detailed walkthrough of the
development of a metamodel for a commonly used modelling language:
DFD's. DFD's were widely used in the 1980's and early 1990's as a
notation for modelling the flow of data between entities in a
system. Indeed they are still used today by data modellers as an
important tool for eliciting data structures. DFD's are a good
starting point for illustrating metamodelling as they are simple,
but illustrate many facets of the metamodelling process.

We begin by giving an overview of DFD's and then follow the
chapters in the book in the development of a metamodel, starting
with the construction of an abstract syntax model, an executable
semantic model, and a concrete syntax model. The resulting
metamodel will be sufficiently rich enough to support the
construction of DFD models both graphically and textually. It will
also have a fully operational semantics, enabling DFD models to be
executed by the XMOF virtual machine. In short, a complete tool
description.

\section{Overview}

As shown in figure \ref{dfdexample}, a DFD is essentially a visual
network of data flows between processes, data stores and external
entities, which aims to model the logical flow of data in a system
and the transformations that occur to the data (without committing
to physical implementation details).

\begin{figure}[htb]
\begin{center}
\includegraphics[width=13cm]{CaseStudy1/figures/DFDExample.pdf}
\caption{An example of a data flow diagram (DFD)}
\label{dfdexample}
\end{center}
\end{figure}

There are a number of other features of DFDs that are not
illustrated by this example. One of the most important is the
ability for processes to be nested. As shown in figure
\ref{dfdnested} ,this enables a single process node on a high level
diagram to be expanded to show a more detailed collections of
processes. The highest level process in the DFD hierarchy is
commonly called a context diagram. This provides a view of the
system as a single process, along with the input and output
dataflows that flow to and from the external entities to the
system.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=13cm]{CaseStudy1/figures/DFDContext.pdf}
\caption{A nested DFD} \label{dfdnested}
\end{center}
\end{figure}

Processes can be decomposed to any level of detail. The diagram in
figure \ref{addreader} shows the decomposition of the NewReader
process.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=13cm]{CaseStudy1/figures/AddReader.pdf}
\caption{Decomposing the NewReader process} \label{addreader}
\end{center}
\end{figure}

Finally, in order to describe the effect of a leaf process, DFDs
typically provide a simple action language. This can be a
specification style language, such as Pspecs \cite{}, which
describes the effect of the process in terms of pre- and post-
conditions, or it can be an operational language. Because we
ultimately wish to be able to execute the DFD's, the latter has
been chosen.

The action language supports a collection of simple actions for
updating and reading records from datastores, making choices, and
calling other actions in other processes.


\begin{lstlisting}
@Process AddReader(name)
  @When
    not Readers.records->exists(reader | reader->at(0) = name)
  do
    @Block
      @Update Readers with Seq{name} end
      @OCLExp "ReaderAdded" end
    end
  end
end
\end{lstlisting}
The action illustrated here is a When action, which has a
condition, that, if true, results in the activation of the action
in the do expression. In this case, if no reader currently exists
with the same name in the Readers datastore, a sequential Block
action is called. This firstly updates the Readers datastore with a
sequence containing the name of the reader and then produces the
OCL string expression, "ReaderAdded".

\section{Abstract Syntax}

\subsection{Identification of Concepts}

Based on the example shown in figure \ref{dfdexample}, the
following candidates for concepts can be immediately identified:

\begin{description}
\item [Process]  A transformer of information that resides within
the bounds of the system to be modelled. Processes appear as named
circles in a DFD.

\item [External Entity] A producer or consumer of information that
resides outside the bounds of the system to be modelled. An external
entity is drawn as a named box.

\item [Datastore] A repository of data records that is to be stored
for use by one or more processes. A datastore is drawn as a half
open box.

\item [Dataflow] Represents the flow of data between processes,
entities and datastores. Dataflows are named and are uni-directional.
Dataflows are shown as lines with a single arrow at one end, pointing
in the direction of the flow.

\item [Action] An action belongs to a process and has a body which
specifies the effect of the action. The following primitive sets of actions are provided:
\begin{itemize}
\item A Send action causes a process in scope to be activated by sending the process a message.
\item An Update action is used to add a record to a data store.
\item A Remove action removes a record from a datastore.
\item An Or action performs a number of actions in sequence until one of them succeeds.
\item A When action allows actions to be activated provided a condition holds.
\item A Block action contains a sequence of sub-actions, which are activated in order.
\item An OCLExp action that contains an XOCL expression which can be evaluated in the normal way.
\end{itemize}

\end{description}

Figure \ref{dfdannotated} shows the same DFD model 'marked up' with
some of the identified concepts. A similar exercise can be carried
out for elements in the action language example.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=13cm]{CaseStudy1/figures/DFDAnnotated.pdf}
\caption{An annotated example of a data flow diagram (DFD)}
\label{dfdannotated}
\end{center}
\end{figure}

\subsection{Abstract Syntax Model}

Once some candidate concepts have been identified, the next step is
to construct an abstract syntax model.

An important question to ask at this point is whether each concept
is an appropriate abstract syntax concept. Datastores, processes
and actions are clearly core to DFDs, as they capture the central
concepts of data and data transformation. There is a question mark
however over external entities and data flows:

\begin{itemize}
\item External entities are external to the system being modelled,
and would appear to be redundent in the sense that they only add
contextual information.
\item Dataflows appear to be derived concepts, as they could be thought
of as showing information flow dependencies between processes and
datastores as the result of actions. For instance, a flow from a
process to a datastore can be derived from an action belonging to
the process that updates the datastore.
\end{itemize}

\noindent For now, these two concepts will be put to one side
\footnote{They will be considered further in the concrete syntax
chapter}.

By focusing on processes, datastores and actions, the model shown
in figure \ref{dfdabs1} is obtained.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=10cm]{CaseStudy1/figures/DFDAbs1.pdf}
\caption{An abstract syntax model for DFDs} \label{dfdabs1}
\end{center}
\end{figure}

There are a number of points to note about the model:

\begin{itemize}
\item Processes are associated with: the collection of datastores that
are accessible by the process; a single action body; and the collection
of sub-processes belonging to the process. A process has a single 'argument'
that it uses to refer to input messages. The body of the process provides
its output messages.
\item Datastores contain an attribute, fields, which defines the names
of the elements in each of its records.
\item Any element that can be viewed as a component of a process is a
specialisation of the class ProcessComponent. This provides an abstract
operation, addTo(), which defines how a component adds itself to a process.
\item {\it When} expressions are associated with a collection of clauses,
which define the rules for testing whether the body of the clause should
be activated.
\end{itemize}

\subsection{Well-formedness Rules}

Whilst most of the concepts and relationship in the DFD language
have been identified,  there are some important rules missing about
what constitutes a well-formed DFD. Firstly, it must be the case
that sub-processes and datastores associated with a process have
unique names:


\begin{lstlisting}
context Process @Constraint AllProcessesHaveUniqueNames
  processes->forAll(p1 |
    processes->forAll(p2 |
      p1.name = p2.name implies p1 = p2))
end

context Process @Constraint AllDataStoresHaveUniqueNames
  dataStores->forAll(p1 |
    dataStores->forAll(p2 |
      p1.name = p2.name implies p1 = p2))
end
\end{lstlisting}
Finally, there are some rules relating to nesting:

\begin{enumerate}
\item There should be no cyclic nesting of processes. This is
required in order to avoid there being cyclic dependencies in a DFD.
\item Sub-processes must only have access to datastores that
are accessible by their parent processes.
\end{enumerate}

\noindent These rules can be expressed as follows:


\begin{lstlisting}
context Process @Constraint NoCyclicDependencies
  not self.allOwnedProcesses()->includes(self)
end

context Process @Constraint DatastoresAreInherited
   datastores->includesAll(processes.datastores)
\end{lstlisting}
\noindent Where the definition of the operation allOwnedProcesses()
is given by the following OCL expression:


\begin{lstlisting}
context Process @Operation allOwnedProcesses():Set(Process)
  processes->
    collect(p | p.allOwnedProcess())
end
\end{lstlisting}
\subsection{Operations}

The following operations are defined for a process:


\begin{lstlisting}
context Process @Operation addTo(p:Process)
  p.addProcess(self)
end

context Process @Operation addStore(store:DataStore)
  self.dataStores := dataStores->including(store)
end

context Process @Operation addProcess(process:Process)
  self.processes := processes->including(process)
end
\end{lstlisting}
The operation addTo() adds a process as a sub-process to the
current process by calling the addProcess() operation. The
addStore() operation adds a datastore to the collection of
datastores that are accessible by the process.

The operation addTo() is similarly defined for a datastore:


\begin{lstlisting}
@Operation addTo(p:Process)
  p.addStore(self)
end
\end{lstlisting}
As we shall see in chapter ??, these operations will become useful
when populating DFDs during parsing.

\subsection{Validating the Metamodel}

In figure \ref{dfdsnapshot} a partial object diagram corresponding
to the DFD in figure \ref{dfdexample} is shown. Here, instances of
XOCL expressions are the values that are passed as expressions to
the actions. The main point to note about this diagram is that it
satisfies the well-formedness rules of the DFD.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=10cm]{CaseStudy1/figures/DFDsnapshot.pdf}
\caption{An object diagram corresponding to figure
\ref{dfdexample}} \label{dfdsnapshot}
\end{center}
\end{figure}

However, this is about as far as we can go. At this point, the
model is just a model of the abstract syntax and nothing more. To
enable DFDs to be conveniently inputed, parsed and executed both
the concrete syntax and semantics of the language must be modelled
too. These aspects will be explored in the following chapters.

\section{Semantics}

Once the abstract syntax model has been completed, the next step is
to define a semantics model, which allows the following:

\begin{itemize}
\item The creation of process instances
\item The creation of datastore instances
\item The execution of a process, with the result that it will evaluate
the action expression to either update a datastore with a value,
remove a value from a datastore, or call another process
\end{itemize}

\subsection{Extending the Metamodel Architecture}

The first step in the process is to identify where the new language
is to  be placed in the metamodel architecture.

There are two places where the DFD model can be viewed as an
extension.  Firstly, a process can be viewed as being a special
type of classifier that defines its own version of new(). What this
means is that a process is like a type, and one can create many
instances of the same type

This enables the creation of new instances of a process.

In addition, processes will also inherit the ability to define
constraints, thus enabling well-formedness constraints on processes
to be written.

Secondly, there is the need to associate a number of actions with
machinery for evaluating expressions. This is the case for Remove,
Update, Send, Clause and OCLExp, which currently say nothing about
the expressions they must evaluate. For example, Update has the
name of the datastore it will update, but also needs to reference
an expression that will be evaluated to produce a result. The
result will be the value used to update the datastore.

To address this, each of the actions are associated with the
Performable class. As mentioned in section ??, the class
Performable is the root of all expressions in XMOF. All subclasses
of Performable must provide the operation eval() in order to state
how to evaluate an expression in the context of an environment. The
resulting model is shown in figure \ref{dfdabs2}.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=12cm]{CaseStudy1/figures/DFDAbs2.pdf}
\caption{Abstract syntax model for DFDs} \label{dfdabs2}
\end{center}
\end{figure}

Note, the advantage of extension here is that ...

\subsection{Concrete Syntax}

\subsection{Semantic Domain}

In order to capture the semantics of process and datastore
instantiation, a semantic domain model needs to be constructed.
This is shown in figure \ref{dfdsem}:

\begin{figure}[htb]
\begin{center}
\includegraphics[width=12cm]{CaseStudy1/figures/DFDSem.pdf}
\caption{Semantic domain model for DFDs} \label{dfdsem}
\end{center}
\end{figure}

Now it possible to define what it means to create a new instance of
a process and a datastore. For a process, the following operation
is required, which is then called from the new() operation:

\begin{lstlisting}
context Root::DFD::Syntax::Process
  @Operation nestedNew(env:Element):Element
    let process = DFD::Semantics::Process.new();
        myProcessEnv = processes->collect(p |
          Seq{p.name})->asSeq; myStoreEnv = dataStores->collect(s |
            Seq{s.name})->asSeq
    in process.definition := self;
       process.processes := processes->collect(p |
         p.nestedNew(myProcessEnv + myStoreEnv + env));
       process.dataStores := dataStores->collect(s |
         s.new());
       @For pair in myProcessEnv do
         pair.tail := process.getProcess(pair->head)
       end;
       @For pair in myStoreEnv do
         pair.tail := process.getStore(pair->head)
       end;
       process.env := myProcessEnv + myStoreEnv + env
    end
  end
\end{lstlisting}where getProcess() and getStore returns the sub-processes and
stores associated with the process.

\section{Conclusion}


==> CaseStudy3/programmingold <==
\chapter{Case Study 3: A Programming Language}

\subsection{Language Definition Example}

The following example illustrates how XOCL it can be used to write
a small interpreter for an expression language that supports
constants, boolean expressions and variables.

A model of the expression classes is shown in figure
\ref{expressions}.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=7cm]{Programming/figures/Expressions.pdf}
\caption{Expression language classes} \label{expressions}
\end{center}
\end{figure}

The result of evaluating an expression is a value. Three types of
values are supported: Integer, Boolean and String values as shown
in figure \ref{values}.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=6cm]{Programming/figures/Values.pdf}
\caption{Value classes} \label{values}
\end{center}
\end{figure}

Boolean values support two operations: boolean `and' and boolean
`or', which return the result of and'ing or or'ing the boolean b
with the boolean value:


\begin{lstlisting}
@Operation binAnd(b)
  Bool(value and b)
end

@Operation binOr(b)
  Bool(value or b)
end
\end{lstlisting}


Integers support the operation `+', which returns the result of
adding the integer i to the integer value:


\begin{lstlisting}
@Operation binAdd(n)
  Int(value + n)
end
\end{lstlisting}


A small interpreter is constructed by defining an eval() operation
on each expression. An eval() expression takes an environment,
env, which is a table of names and values that correspond to the
bound variables in scope when the expression is evaluated.

The eval() operation for boolean expressions evaluates the left
hand boolean expressions with the right hand boolean expression:


\begin{lstlisting}
context BoolExp
  @Operation eval(env)
    @Case op of
      "and" do left.eval(env).binAnd(right.eval(env)) end
      "or"  do left.eval(env).binOr(right.eval(env)) end
      "+"   do left.eval(env).binAdd(right.eval(env)) end
    end
  end
\end{lstlisting}


Evaluating a constant expression will create an instance of the
appropriate value depending on the type of the expression's value:


\begin{lstlisting}
context Const
  @Operation eval(env)
    @TypeCase(value)
      Boolean do Bool(value) end
      Integer do Int(value) end
      String  do Str(value) end
    end
  end
\end{lstlisting}


Finally, evaluating a variable expression simply looks up the
value of the bound variable:


\begin{lstlisting}
@Operation eval(env)
  env.lookup(name)
end
\end{lstlisting}


==> LanguageDrivenDevelopment/ldd.ibm.tex <==
\chapter{Model-Driven Development}
\label{mddchapter}



\section{The Future of Software and Systems Engineering} \label{futureengineering}

\subsection{Managing Complexity Is Not Enough} \label{complexityanddiversity}

This being a software and systems engineering book, we feel duty bound to start with something along the following lines:

\begin{quote}
The theories, methods and tools of software and systems engineering bring a discipline to the development process that enable the increasing complexity of today's systems to be managed in a rigorous and scalable manner.
\end{quote}

This also being a software and systems modelling book, we feel obliged to carry on with something like this:

\begin{quote}
Software and system modelling is the latest step in a continuing trend of increasing abstraction in system development, allowing us to move further away from the low-level implementation-oriented viewpoint towards the high-level problem-oriented viewpoint.
\end{quote}

So is that it? Is modelling the means of coping with the problems of modern software and system development? The anwser to the latter question is an unequivocal "yes!", but not in the way it is currently being applied. The plight facing today's developers is not simply one of complexity (although this is bad enough) - there are many other factors to contend with. This chapter investigates the true nature and needs of modern software and system development, and proposes an approach that is in tune with those needs.

So no, the above soundbites certainly are not "it".

\subsection{Managing Diversity: The New Software Crisis?} \label{diversity}

Before we start to talk about model-driven anything, we need to clarify what the problems are that we're trying to solve. Here are some problems commonly faced by developers today:

\subsubsection{Diverse Domains}

The requirements of large systems often relate to a variety of domains that need to be reconciled by different stakeholders. These requirements may range far and wide, including functional, safety, security and performance considerations. Each domain often has its own specialist approach for dealing with appropriate requirements requirements, but their specialist nature inevitably precludes them from being applied in other domains.

\subsubsection{Diverse Customer Requirements}

The 'one size fits all' approach to software and systems is increasingly inappropriate in today's market. Vendors who offer products that can be tailored to the specific needs of a customer have a strong commercial advantage, but developing products that are truly customisable such that they can meet the demands of a broad customer base is a far from trivial matter. Despite the fact that two products being offered to different customers may share significant functionality, large rewrites and redesign are often required because the functional components of a system are too tightly coupled to allow large scale reuse. In addition, many systems are designed at too lower level of abstraction to yield optimum flexibility.

\subsubsection{Diverse Implementation Technologies}

Systems often need to be deployed across different implementation technologies, each of which have their own requirements and languages. However, the separation between the core functionality and the requirements of the deployment platform is rarely kept clean during the development of the system. It has been recognised that in order to support redeployment (or indeed other customisation such as described above), systems need to be designed at a high level of abstraction; thus software and system modelling has become popular, but these models are rarely complete. Software models in particular seldom get beyond the specification of their behaviour, such that code cannot be completely generated. Even when code is generated, full testing and validation is usually required, and that is a significant chunk of development effort.

\subsubsection{Diverse Tools and Artefact Types}

During the development of a system, a large number of artefacts are created, including requirements specifications, design documentation, design and analysis models, analysis and simulation data and of course the code (for software systems). Unfortunately, these artefacts are often prevented from being truly valuable assets because:
\begin{itemize}
\item they are often created by different incompatible tools or using different languages, some of which may no longer be supported, such that the artefacts become unmaintainable;
\item the forms of artefacts are incompatible, and many are written in informal languages, such that there is no clear way to integrate the information they contain;
\item artefacts such as design models are rarely kept in step with changes to the implementation artefacts such as code, because there is no automatic way to do, vastly reducing their value as assets;
\item the artefacts that are kept up to date, such as code, are often tightly coupled to the integration technology, reducing their value as reusable assets;
\item many artefacts only exist on paper rather than electronic form, so any maintenance or integration tasks has to be manually.
\end{itemize}
This may be fine for one-off stable systems, but systems are rarely built from scratch - they are often based on existing systems, and as such would ideally reuse as much as possible from the baseline system. Similarly, nearly all systems evolve, and code is not always the ideal starting point for managing change.

\vspace{1cm}
\noindent
All the above point to diversity as the new major problem facing developers today. Modelling has certainly helped to manage complexity by raising the level of abstraction, but does not in itself tackle the problem of diversity. One way of tackling it is to try to stem the flow of diversity itself by finding a common language with which developers can model their systems - section \ref{uml} charts one well-known valiant but ultimately doomed attempt at this. The other alternative is to go with the flow and embrace the full multi-coloured tapestry of diversity head-on. This is where true Model-Driven Development (or MDD) differs from common or garden modelling. Simple modelling has the weapon of abstraction to wield, but Model-Driven Development adds the weapon of languages.


% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = =


\section{The Vision of Model-Driven Development} \label{mddvision}

\subsection{Languages are the Future}

Section \ref{diversity} highlighted how diversity lies at the heart of modern system development. Going a step further, we suggest that the challenge really boils down to a diversity of languages:
\begin{itemize}
\item specialists require languages to address the particular facets of the problem that lie within their domain - often within each specialist domain there are numerous languages, with new languages being developed all the time;
\item there are countless implementation languages - some differences are due to the continuing trend of increasing abstraction, some are due to the fact that different paradigms or individual languages are better suited to a particular problem-solution pair than others, and some are simply down to competitive commercial interests;
\item the languages and syntax that capture the artefacts created during the development lifecycle.
\end{itemize}

If a development process limits itself to the application of a fixed set of languages, it will necessarily limit the range of problems that it can address as well as the potential solutions it can provide. Instead, a development process should incorporate the ability to adopt and construct whatever languages provide the best fit. In other words, there should be a shift in emphasis from system development to language development.

One could argue against this by saying that Turing and Church demonstrated that everything can in fact be boiled down to constructs in a very simple language, but this is a theorist's argument. Whilst it is technically feasible, any gain made in widening the applicability of a language to different domains will be at the expense of the richness of the language that makes it so suitable for a particular domain (section \ref{uml} describes some of the pitfalls of this approach in more detail). However, in a very real sense, the concept of a single small underlying language provides the basis for realising Model-Driven Development. This is the domain of metamodelling, and is the topic of Chapter \ref{metamodellingChapter}.

It is important to clarify what we mean by the term 'language' here. Section \ref{syntaxsemantics} describes the features and components of languages in detail, but there are two important points to make here in the context of Model-Driven Development. Firstly, in order to be useful, a language should be a precise and unambiguous formalism - in other words, there should be clear rules which dictate what does and does not constitute a valid application of the language. Without this, any form of rigourous analysis, testing or transformation becomes impossible. Secondly, a language must have meaning (also known as semantics) as well as form (also known as syntax). Any formalism which has no meaning is a notation rather than a language. Notations have their part to play in MDD, but it is important to realise that by definition, in order to have meaningful models, the language in which they are described must have a semantics. In addition, just as with syntax, in order to be useful in an MDD context, the semantics must be precisely defined. These points may seem obvious, but in fact, many formalisms which are currently used for system and software modelling can really only be described as notations rather than languages - this severely limits the potential power that these formalisms can yield in the MDD world.


%Productivity can be increased because engineers and domain experts can speak in the languages they understand, and both the problem space and solution space are opened up to their full extent. [This approach could potentially offer a layer/ paradigm shift above OO programming that could have major implications in terms of productivity, etc to industry. (Andy e-mail)]


\subsection{Language Integration}

%language islands
%proof: lots of dsl's - argument that there only not more of them because language islands don't work

\subsection{Requirements of MDD} \label{mddreq}
%Problem-driven not technology-driven (James)
%Customers: industrial-based systems and software engineers


% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = =


\section{Current State of Model-Driven Development} \label{mda2mdd}

\subsection{The Unified Modelling Language} \label{uml}

%Trying to have a single homogenous language doomed

%Books such as [] implicitly suggest that a broad range of problems can be solved by a set of languages X, Y and Z (UML, OOA, Booch...). Having said this, the inability of languages such as UML (in its vanilla form) to support tasks such as the engineering of real-time systems, for example, has led to "real-time" extensions to that language via profiles (we shall avoid discussing the limitations of profiles as a language definition mechanism at this stage). But if one is to examine the number of types of requirements faced by real-time systems developers, it is impossible for one language however well designed to anticipate them all. Moreover, the act of trying to design a language which anticipates all possible uses invariably gives rise to a language which is large, difficult to understand and difficult to apply. (This claim is reinforced in the context of real-time systems when one examines the literature which introduces new mechanisms week by week catering for new types of requirements). - James' paper

%Need to outline benefits as well as pitfalls - single language is easier to roll out across developers etc. (Andy)

Modelling has been used in software engineering since its inception, but most methodologies proposed over the years have included their own particular modelling notation and tools, which made model interchange difficult. This invariably led to a situation where software developers were locked into a particular tool vendor that supported a particular methodology \cite{umllrm}. In the nineties, after an influx of object-oriented methodologies such as Schlaer-Mellor \cite{schlaermellor}, Coad-Yourdon \cite{coadyourdon} and OMT \cite{omt}, the Object Management Group \cite{omg} (OMG) instigated a drive to unify the variety of modelling notations (rather than the methodologies), which were seen to share a lot of common concepts.

The result was the Unified Modelling Language (UML)\cite{umlspec}, which was adopted in November 1997. UML consists of a number of different notations that allow different views of a software system to be modelled at different stages of the development lifecycle. Both static and dynamic aspects of a system can be captured, and facilities are also provided to enable model management and limited extensibility (described in more detail in section \ref{???}. A textual constraint language (OCL) is included to allow the state space represented by a model to be further constrained in ways that are too complex to be captured by the graphical notations alone. The UML views and notations are summarised in Table \ref{tableuml}.

\begin{table}[htb]
\begin{center}
\includegraphics[width=14.5cm]{ModelDrivenDevelopment/figures/tableuml.pdf}
\caption{\textbf{UML Views an Diagrams.} \em{Based on \cite{umllrm}.}}
\label{tableuml}
\end{center}
\end{table}

UML has been well-received and is now the \emph{de facto} software modelling language, but it is not without its shortcomings. The three main areas for concern with UML 1.x, which have led to the development of UML 2.0 and MDA, are listed below and described in detail in the remainder of this section:
\begin{itemize}
\item the definition of the language itself is incomplete, imprecise and incoherent;
\item the language is not flexible enough to support the wide range of potential domains;
\item it is not executable.
\end{itemize}

\subsubsection*{Imprecise semantics}

Section \ref{model} explained the importance of unambiguous models within engineering disciplines, and that in order to achieve this, modelling languages must have a precise semantics. The specification for UML 1.x\cite{umlspec} falls some way short of this - whilst its syntax is mostly well specified, the semantics of those syntactic elements is either missing or provided informally using English. This has led to a situation where, as of version 1.3, no tool could claim to UML compliant \cite{pumlrfi}. This in turn has inhibited model interchange between tools, leading back to the situation of vendor lock-in. In addition, as explained earlier, models written in such an informally specified language are open to misinterpretation, a potentially dangerous or expensive problem. Whilst a major revision of UML will be released soon, draft versions of the UML 2.0 standard do not indicate major improvements with regard to semantics.

\subsubsection*{Limited scope and flexibility}

UML has been successfully applied across the software development community, and it is increasingly being applied to non-software domains such as systems engineering\cite{umlse}, and specialised software domains such as real time and high integrity systems. The diverse modelling requirements that this widespread use brings makes defining what a unified modelling language should be a considerable problem. Early attempts to enhance UML to support new requirements adopted a 'mud-packing' approach\cite{kobryn}, which involved making direct amendments to the monolithic definition of UML itself. This resulted in a language that became increasingly large, unwieldy to use, incomprehensible, and difficult to maintain and test for consistency.

In order to overcome these problems, UML was refactored from a one-size-fits-all modelling language into a family of languages. The foundation of the UML family is a stable core UML metamodel, consisting of minimal modelling concepts that are supported by all family members. Each dialect of UML consists of the UML core metamodel and one or more extensions to the core known as `profiles'. The UML 1.4 profile mechanism is quite straightforward to apply, but is limited as it is based upon constraining existing language constructs rather then modifying or adding new language constructs. The profile mechanism offered by UML 2.0 promises to be more powerful, allowing direct extensions to the language constructs - this is obviously an important step forward. However, it would be naive to think that every possible domain could be modelled using a profile of UML. If nothing else, the UML core is still fundamentally object-oriented, which is quite a problem for non OO domains. Thus in some cases, it is necessary to define modelling languages that are quite independent of UML. How models written in these seemingly disparate languages are integrated into a unified process is the subject of MDA (see section \ref{mdavision}).

\subsubsection*{Non-executability}

*** TO BE FINISHED ***

%action semantics
%executable UML

\subsection{MDA}
%PIMs to PSMs too limited
%MOF not powerful enough
%Architecture not flexible enough
%Too driven by tool-vendors - vaguely defined marketing banner that they can flog their products under

MDA is an ambitious vision that could change the way software is developed in the future. However, there are some limitations to MDA that need to be considered:
\begin{itemize}
\item MDA does not specify the way in which mappings should be realised. A true Model Driven Software Development process would realise mappings as models, as this would bring all the benefits of modeling and allow similar tools to be applied to mappings as other models. It would also allow mappings themselves to be transformed \cite{bezivinmda}.
\item MDA is too fixed on the notion of \emph{platform}. The answer to what constitutes a \emph{platform} is unclear at best - the transition from the most abstract model of a system to the most refined model may include several stages of models, each which could considered Platform Specific when compared to the previous stage, or Platform Independent when compared to the following stage. Also, mapping models or language models as well as system models may be transformed - here the notion of platform makes less sense. Instead, the broader notion of Model Driven Software Development is just concerned with models and mappings.
\item The four layer metamodel architecture of Figure \ref{figmetamodelarch} is quite inflexible, because it arbitrarily limits the number of levels of instantiation \cite{panhorrocks}, enforces a type distinction between models at different layers and does not support the modeling of the instantiation relationship (since they exist outside of all the levels). These and other architectural issues are detailed in section \ref{archprobs}.
\end{itemize}

%Andy Key that we get across that MDD is not just about PIM to PSM mappings it is about being able to capture all aspects of the systems development process etc in a unified way, and all the benefits that brings to developers.

\subsection{QVT}


% = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = = =


\section{Conclusion}
%Complexity AND diversity
%Languages are the new OO
%Mappings
%Integration of artefacts written in different languages - next chapter introduces a means of doing this
%Introduction to rest of book





%*** Andy's Metamodelling chapter ***
%2.0: The previous chapter described how model-driven development is fundamentally based on the use of modelling languages to capture and relate different aspects of the problem domain. These languages may be general purpose languages like UML or domain specific languages such as XML.
%2.1.4: In the real world, modelling languages do not exist in isolation. They will always be related to other languages.


==> MetaToolArchitecture/kernel.tex <==
\chapter{A Meta-Tool Architecture}
\label{kernelchapter}

\section{A Metamodelling Kernel}

The previous part of the book has shown how a rich metamodelling language such as XMOF allows the description of complex languages.  XMOF is a language and like any other language has a semantics.  If its semantics are not well understood then the rigour of any language defined using XMOF is compromised.  Up until now, questions of XMOF's semantic soundness have been avoided, instead informal descriptions of the constructs have been given.  This part of the book examines the semantics basis of XMOF in more detail and demonstrates how its semantics can be described in terms of the kernel language core-XMOF (a subset of XMOF itself).

% Even if the semantics of XMOF are described in terms of some other language, an obvious (recursive) question is - what should that language be defined in terms of?  Often the ultimate language is mathematics because of its universally consistent interpretation.  But mathematical descriptions of even simple languages can often be quite verbose and unpalatable to non-mathematicians.  Another option is to treat an implementation of a language as its semantic basis.  This approach is commonly used by programming languages such as Java and C++.  If a programmer wishes to understand the semantics of a particular program language construct, a program can be written which uses the construct and the resulting behaviour observed.

%In this chapter the former approach is taken.  However, rather than using mathematics the preference is to make core-XMOF so simple that the semantics can be understood from informal descriptions.  Using the informal descriptions of core-XMOF it is a short step to creating a programming-language-like machine which can interpret the kernel.  This would effectively be a virtual machine for XMOF.

\section{The Language Tower}

The first part of the book demonstrates how metamodels can be built using XMOF as a base language.  By virtue of being a language, XMOF must be an instance of some other language, that language is core-XMOF.  This kind of architecture gives rise to the language tower an example of which is illustrated in figure \ref{tower} (a).

There are two related issues with the tower of \ref{tower} (a).  Firstly the need to define XMOF in terms of a further language begs the question, what language should that further language be defined using?  This question is recursive because languages can be continually inserted at the foundation of the tower without ever bottoming out.  The second issue is that there are several different types of layers within the example tower of figure \ref{tower} (a):

\begin{figure}[htb]
\begin{center}
\subfigure[An illustration of a language tower]{\includegraphics[width=4cm]{MetaToolArchitecture/figures/tower1.pdf}}
\subfigure[Introducing uniformity into the tower by making the bottom layer self defining]{\includegraphics[width=3.8cm]{MetaToolArchitecture/figures/tower2.pdf}}
\caption{Language towers}
\label{tower}
\end{center}
\end{figure}

\begin{itemize}
\item Layers which are model instances (aDFD).
\item Layers which are instances and are models for instances (DFD).
\item Layers which are instance, models and metamodels for instances (XMOF).
\item Layers which are metamodels only (core-XMOF).
\end{itemize}

\noindent Although this may not seem problematic, the lack of uniformity in the architecture makes it complicated to define.  In a larger tower most layers would conform to that of XMOF in the sense that they would be an instance, model and metamodel.  As with the first issue, the problem rests with the base layer (core-XMOF) which is distinct from the other layers in that it is not an instance of any other language.

A solution to this problem is described in \cite{objVlisp} and involves making the base layer self defining as illustrated in figure \ref{tower} (b).  This solves the first issue mentioned because every layer is now an instance.  The self dependency also provides a much greater level of uniformity because there are fewer types of layers to consider:

\pagebreak
\begin{itemize}
\item Every layer is an instance;
\item a layer can be a model for instances;
\item or, a layer can be a model and metamodel for instances;
\end{itemize}

The architecture exemplified in figure \ref{tower} (b) is used as a basis for core-XMOF which will be described in the remainder of this chapter.  Despite the self defining nature of core-XMOF, it is important to recognise that an external language is still required to define core-XMOF.  The self defining nature creates a closed world for creating languages, this world is elegant because it requires few semantically distinct concepts in order to realise it.  Because there are fewer concepts, this also reduces the dependency on the world outside of core-XMOF, but that world must still exist.  This effectively gives rise to a towers-within-towers architecture an example of which is illustrated in figure \ref{towerOfTower} where the core-XMOF tower is defined using C++.  It is interesting to note that all concepts within a tower can be viewed as instances of the containing tower.  In the case of figure \ref{towerOfTower} the core-XMOF based languages can be viewed as an instances of C++.

Programming languages are a good way of defining core-XMOF because the result is a machine that will interpret languages constructed from core-XMOF and the imperative aspects of core-XMOF will execute.  From the point of view of comprehending the semantics of a language, this is advantageous because the semantics of a particular construct can be understood by executing an instance of that construct.  For the purpose of presenting semantics on paper it is less than ideal because many mechanisms must be introduced which are superfluous to the essence of the semantics, these are there to \emph{make the implementation work} in a particular programming language.

An alternative approach is to ground the kernel in a non executable language which has a universal consistent interpretation such as maths.  But mathematical descriptions of even simple languages tend to be quite verbose and unpalatable to non-mathematicians.  For this reason, this chapter resorts to explaining core-XMOF informally.  Although informality is never ideal, it is perhaps more appropriate in the case of core-XMOF because, as has been previously explained, core-XMOF has few distinct concepts.  Using the informal descriptions it is a short step to creating a core-XMOF programming-language-like machine which can interpret the kernel.  Details of how to implement interpreters for similar languages in Java can be found in \cite{programLanguageProcessors}.


\begin{figure}[htb]
\begin{center}
\includegraphics[width=12cm]{MetaToolArchitecture/figures/towerOfTower.pdf}
\caption{A language tower containing another language tower}
\label{towerOfTower}
\end{center}
\end{figure}

\section{Building the Tower}

Having simplified the language tower framework, it is now necessary to understand how to build such a tower.  To recap the requirements for the tower are: every layer is an instance, a layer can be model for instances or, can be a model and metamodel for instances.  One object oriented approach that provides a concise framework for addressing these requirements can be found in \cite{objVlisp}.  In this there are two class:

\begin{itemize}
\item Class: defines a model for instances which are the basis for further instances (a metamodel).
\item Object: defines a model for instances (a model).
\end{itemize}

\noindent Using these classes in two different configuration enables the requirements listed above to be dealt with.  An example of the first configuration is illustrated in figure \ref{core2}.  In this \emph{Animal} is a model because it is an instance of \emph{Class}, and is an instance itself because \emph{Class} inherits from \emph{Object}.  \emph{Chicken} and \emph{Dog} are instances because \emph{Animal} inherits from \emph{Object}.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=9cm]{MetaToolArchitecture/figures/core2.pdf}
\caption{Defining instances who instances are terminal (models)}
\label{core2}
\end{center}
\end{figure}

An example of the second configuration is shown in figure \ref{core3}.  Here \emph{Statemachine} is the basis for further instance because it is an instance of \emph{Class}, and is an instance itself because \emph{Class} inherits from \emph{Object}.  Because \emph{Statemachine} inherits from \emph{Class} then instances of \emph{Statemachine} can also be the basis for further instances.  \emph{Statemachine} is an object because it is an instance of \emph{Class} which inherits from \emph{Object}.  \emph{Switch} is an object because it is an instance of \emph{Statemachine} which inherits from \emph{Object}, and \emph{Switch1} and \emph{Switch2} are objects because they are an instance of \emph{Switch} which inherits from \emph{Object}.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=10cm]{MetaToolArchitecture/figures/core3.pdf}
\caption{Defining instance who instances can have instances (metamodels)}
\label{core3}
\end{center}
\end{figure}

Figures \ref{core2} and \ref{core3} are not however an accurate representation of the self defining language tower since the bottom layer \emph{Class} is not an instance of itself.  This is rectified by introducing the configuration illustrated in figure \ref{core1}, this configuration is often referred to as the \emph{golden braid} \cite{geb} because of the mutual dependencies between its components.  The self defining base level is described by \emph{Class} being an instance of itself.  Note that \emph{Class} is also an object because of it is an instance of \emph{Class} which inherits from \emph{Object}.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=3cm]{MetaToolArchitecture/figures/core1.pdf}
\caption{The self defining configuration}
\label{core1}
\end{center}
\end{figure}

The configuration of \ref{core1} forms the heart of core-XMOF and enables core-XMOF to be used to build language towers.  Although these configuration may seem confusing at first, they are an elegant approach to language architecting because there are few primitive concepts to understand the semantics of (these are effectively instantiation and generalisation).  The semantics of these could be given in some mathematical language, or implemented in a programming language.  As mentioned in the introduction the preference is to treat these concepts as the fundamental language and explain them informally without need for an external system.  In the next section we describe the semantics of core-XMOF in more detail.

\FloatBarrier

\section{Core-XMOF}

In this section the core-XMOF kernel is introduced in more detail. This involves putting `meat on the bones' of the configurations described in the previous section and more concretely describing the mechanics of the kernel.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=8cm]{MetaToolArchitecture/figures/moreDetail.pdf}
\caption{The self defining configuration in more detail}
\label{moreDetail}
\end{center}
\end{figure}

Figure \ref{moreDetail} illustrates the Class/Object configuration once again but this time augmented to include their slots.  Class has four slots \emph{name}, \emph{parents}, \emph{attributes}, \emph{operations} and \emph{of} (\emph{parents} is depicted diagrammatically by the inheritance arrow).  The slots of an object correspond directly to the attributes of the object's class.  In the case of Class, its slots are the union of the attributes of Class and Object (because of the inheritance relationship).  The direct correspondence between a Class's attributes and slots is what makes Class self defining.

When an operation is invoked on an object, the operation lookup protocol navigates to the object's class in order to find the appropriate operation.  The means by which objects are instantiated is specified by the \emph{new} operation in Class, this operation is special because it is one of two operations whose semantics are specified outside of the kernel.  The semantics of \emph{new} have been hinted at already and involve a number of steps:

\begin{itemize}
\item Calculating the union of the class's attributes and the attribute's of the class's parents.
\item Creating a new object with slots corresponding to each of the class's attributes.
\item Setting the value of the \emph{of} slot to that of the class responsible for the instantiation.
\end{itemize}

\noindent A further example of this is shown in figure \ref{moreDetailExample2} where the class \emph{Animal} has a set of attributes defining \emph{name}, \emph{noLegs} and \emph{barks}.  The resulting object has slots for each of these attributes plus \emph{of} since \emph{Animal} inherits from \emph{Object}.

% Operations performed on the class

\begin{figure}
\begin{center}
\includegraphics[width=12cm]{MetaToolArchitecture/figures/moreDetailExample2.pdf}
\caption{An illustration how of how a class's attributes defines the slots of its objects}
\label{moreDetailExample2}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=12cm]{MetaToolArchitecture/figures/moreDetailExample.pdf}
\caption{The self defining configuration}
\label{moreDetailExample}
\end{center}
\end{figure}

\section{Class Diagrams}

Having defined the foundation kernel-XMOF in the previous sections, this section demonstrates how the metamodel for class diagrams can be constructed using the kernel.

\section{OCL and OCL++}

The earlier part of the book demonstrates how OCL and OCL++ are key components in a language engineers armoury.  In this section it is shown how these languages can be metamodelled using the core-XMOF kernel.

\section{Mappings}

If the relationships between metamodels cannot be understood, then the ability to use multiple models to describe systems is of limited use.  Chapter \ref{} illustrates how a mapping can be constructed between two diverse metamodels.  This section grounds the semantics of that mapping language using kernel-XMOF.

\section{Conclusion}


==> Metamodelling/metamodellingold.tex <==
\chapter{Metamodelling} \label{metamodelchapter}

\section{Introduction} \label{metamodelintro}

\section{Defining a Modelling Language} \label{languagedef}

\subsection{Components of a Modelling Language} \label{langcomponents}

%-Modeling Language Requirements and Features
%===========================================
%defining modeling languages comes in section \ref{languagedef}
%no single set of constructs and features that will satisfy all needs -> profiles
%static language used to represent collections of structured data; dynamic language is used to represent executable actions (Tony's `Defining Languages in XMT')
%large scale reuse (templates?) - consistent architecture (for enterprise/system models, business models, metamodels (a.s, c.s., semantics) -> templates can help \cite{mdadsouza}
%constraint language

%make distinction from `features' of a modeling language
%James formal semantics of programming book

%\subsection{Modeling vs. Programming Languages}
%\subsection{Principles of Modeling Language Design}
%\subsection{Formal vs. Informal Semantics} \label{formalintro}
%\subsection{Approaches to Formalising Semantics}
%\subsection{Formal vs. Metamodeling Languages}

\section{Metamodel Architecture} \label{metamodelarch}

\subsection{MOF and the Four-Layer Architecture} \label{mof}

%MDA is not a single technology itself, but a unifying framework for a number of related model-driven technologies and standards, such as UML, the Meta-Object Facility (MOF) and XMI.

%UML has become the \textit{de facto} modeling language since its adoption in 1997, and is used for modeling all aspects of software systems throughout the development lifecycle (the system modeling space). UML is described in more detail in section \ref{mdsdlang}.

%Whilst there are number of ways of defining languages such as UML (see section \ref{languagedef}), in MDA language specifications are themselves models (known as \emph{metamodels}), which are defined as instances of the Meta Object Facility. MOF is a language for specifying technology neutral metamodels and for implementing repositories of metadata \cite{mofspec}. The syntaxes of MOF and UML are quite similar, but because of their different usage scenarios (MOF is used primarily for defining languages, UML for describing systems), they are not totally aligned \cite{mofspec}. The OMG specifies an architecture for relating the various system models and language metamodels, which is depicted in Figure \ref{figmetamodelarch}. The relationship between models at consecutive levels is one of instantiation. Note that the specification for MOF is defined as an instance of itself to eliminate the need for a layer above M3. MOF and the metamodel architecture (particularly the limitations of the four layer architecture) are discussed in detail in section \ref{metamodeling}.

%\begin{figure}[htb]
%\begin{center}
%\includegraphics[width=8cm]{ModelDrivenDevelopment/figures/metamodelarch.pdf}
%\caption{\textbf{The OMG Four Layer Metamodel Architecture.}}
%\label{figmetamodelarch}
%\end{center}
%\end{figure}

%Another important aspect of MDA is that models should be freely interchangeable between tools and repositories, as highlighted in section \ref{mdavision}. In order to enable this, OMG has adopted an interchange standard called the XML Metadata Interchange (XMI) \cite{xmispec}. XML is a syntax for representing structural data in a textual form. The valid structure of a particular set of XML documents can be captured in an XML DTD (Document Type Definition) or schema - any XML document can be then be checked against the appropriate DTD or schema for well-formedness. XMI allows MOF metamodels and UML models to be represented as XML documents. These be checked against the MOF DTD or UML DTD respectively for well-formedness. Because languages other than UML can be defined using MOF, XMI also provides a facility for generating an appropriate DTD for any MOF compliant metamodel, so the well-formedness of instances of that metamodel can be checked.

\subsection{A Reflective Metamodel Architecture} \label{reflection}

\section{Architecture of a Language Metamodel} \label{langarchitecture}

\section{Process for Constructing Language Metamodels} \label{metamodellingprocess}

%need abstract syntax, semantics and interpreter, and THAT's IT!
%reflection?


% LITERATURE REVIEW
%==================

%\section{Metamodeling} \label{metamodeling}

%\subsection{Metadata and Metamodels} \label{metadata}

%data about data - equivalent to models
%MDR - metadata repository
%MOF
%code as model - code does not need to be a UML model but it must be an instance of a MOF metamodel
%data warehousing / CWM
%tools understanding metamodeling language -> customisable; guis as models (see tools above)
%syntax, semantics, constraints, concrete syntax

%Metatools
%=========
%tools understanding metamodeling language -> customisable; guis as models
%mdsd - tools (gui) etc. as models; move away from bespoke
%metatools: MetaEdit+, Dome, PROGRESS (graph grammars), MMT \cite{pumlmda}, KMF, XMT, IBM EMF (EMF.Edit, EMF.Codegen)
%tools should be able to export instances of their models in XMI that is a valid instance of a metamodel (e.g. UML metamodel) (*ANDYBAE*)
%tools should be able to supply info about their metamodel in a form that is a valid instance of an appropriate meta-metamodel (e.g. MOF) (*ANDYBAE*)


%\subsection{Requirements for a Metamodeling Language}

%\subsection{Architectures for Metamodeling} \label{metaarch}

%supposed advantages of fixed metamodel architecture (\cite{mofspec} p.2-3)

%\subsection{Fixed vs. Reflective Architectures}

%\subsection{Architectural Problems} \label{archprobs}

%already outlined in \ref{introarchfix}!
%Instantiation and Meta-instantiation
%problems with kuhne work!
%consistent architecture (for enterprise/system models, business models, metamodels (a.s, c.s., semantics) \ref{mdsdarch}
%nature of metamodel architecture : fixed vs. reflexive, translational vs. extensional approach to semantics; where do semantics live, where do mappings live; how to map different views of UML? what about inter-layer mappings? what about the definition of the architecture itself?
%translational vs. extensional approach? (MOF vs. infrastructure vs. superstructure): "as far as possible, new constructs should be defined by translation to the core, rather than have independently defined semantics" \cite{mdadsouza}
%translation - good: all superstructure maps down onto a simpler domain, and mapping is all at abstract syntax level; bad: information in original model can potentially be lost (Andy e-mail "Re: Superstructure vs. Infrastructure", 19 March 2002)
%models have been used in the software development process for some time, but the resultant models are intermediate artefacts leading to code, rather than valuable artefacts in themselves; failure to unite different views; need to separate meaning from representation;``each of UML's myriad diagrams is then merely a projection of the underlying language specification'' \cite{mellor}


%\subsection{Languages for Metamodeling}

%XMI not rich enough

%\subsection{The OMG's Meta-Object Facility}
%limitations of MOF
%MOF too repository biased. Should be able to model check etc.
%why O-O? (see \ref{oo}). Not just for modeling OO software 

==> XMF/XMOF_with_statemachines.tex <==
\chapter{A Language for Metamodelling}
\label{xmofchapter}

\section{Introduction}

As we saw in the previous chapter, a metamodel should not only be
able to describe the modelling concepts provided by the language
(its abstract syntax), but also many other important features of a
language definition, including semantics  (the meaning of the
language), concrete syntax (how the language is presented) and
other features such as relationship to other languages in the world
around it.

Any metamodelling language appropriate for describing languages
must be expressive enough to capture all these different aspects in
a platform independent way. In other words, the resulting
metamodels should be self sufficient and independent of
implementation specific descriptions of the language being
modelled. Thus, reliance on the implementation of the language's
behaviour in an external programming language, or the assumption
that there will be an external database which manages object
creation and persistence should be completely avoided.

The language presented in this chapter does just this. This
language, which we call XMOF, combines and extends a number of
standard modelling facilities to provide a minimal, but expressive,
platform independent language for metamodelling. XMOF includes the
following features:

\begin{itemize}

\item Support for standard OO modelling concepts such as packages, classes, and
associations to describe language concepts and their relationship to one another.

\item A constraint language, which can used to describe well-formedness rules.

\item A set of action primitives, which can be used to capture the behavioural semantics of a language.

\item A language for expressing mappings between languages and language components.

\item A concrete syntax language which can be extended to support new concrete syntaxes of languages with ease.

\item A generic metamodel framework, which supports standard plug-points and machinery for
expressing model element instantiation, execution, expression evaluation and reflection.

\end{itemize}

\section{XMOF Features}

The following sections present an overview of the key features of
XMOF. This is not a full definition, but will reference fuller
descriptions of the components of the language where appropriate.

\subsection{OO modelling concepts}

XMOF provides the standard OO modelling concepts that are supported
by MOF and UML, including packages, classes and associations.
Traditionally, these are  visualised using class diagrams. Figure
\ref{classDiagram} shows an example of a class diagram of a simple
model consisting of a package with a number of classes and
associations. This model describes a simple state machine, where a
state machine contains states and transitions, and transitions have
source and target states.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=8cm]{XMOF/figures/classDiagramExample}
\caption{An example of a class diagram}
\label{classDiagram}
\end{center}
\end{figure}

XMOF also provides a concrete syntax for packages and classes. The
equivalent concrete representation of the state machine class
diagram shown in figure \ref{classDiagram} is shown below.

\small
\begin{verbatim}
1 @Package StateMachine
2    @Class isAbstract Named
3      @Attribute name : String end
4    end
5    @Class StateMachine
6      @Attribute states : Set(State) end
7      @Attribute transitions : Set(Transition) end
8      @Attribute startingState : State end
9    end
10    @Class State extends Named
11   end
12   @Class Transition extends Named
13     @Attribute source : State end
14     @Attribute target : State end
15   end
16 end
\end{verbatim}

Here, line 1 shows the start of a package named StateMachine, which
contains all the sub-definitions relating to state machines.

Line 2 contains the start of a class definition for the class
Named,  which is an abstract class for a named element. Line 5 is
the start of the definition of the StateMachine class. It defines
two attributes named states and transitions, whose types are
Set(State) and Set(Transition). These types correspond to the "*"
multiplicity of the equivalent association ends in the class
diagram.

Lines 10 and 12 are the start of the State and Transition class
definitions. Both these classes specialise the class Named, and
therefore inherit a name attribute. A Transition has two attributes
source and target, which are of type State. The fact that they are
single valued reflects the multiplicity of the equivalent
association ends in the class diagram.

As chapter \ref{concretesyntax} will show, the concrete
representation  of a modelling language should be clearly
distinguished from its abstract syntax representation. Here, two
different concrete syntaxes are essential being used to capture the
same information.

\normalsize

\subsection{Constraints}

It is often necessary to make well-formedness statements about
concepts in a model.  These statements are often made informally,
for example in the context of figure \ref{classDiagram} it might be
useful to specify that \emph{all transitions have unique names
within a state machine}. A constraint language provides a means of
succinctly expressing complex well-formedness rules unambigiously.
For example the well-formedness statement mentioned above can be
added to the class StateMachine in the following way:

\small
\begin{verbatim}
context StateMachine::StateMachine
  @Constraint NoTwoTransitionsWithTheSameName
    self.transitions->forAll(t1 |
      self.transition->forAll(t2 |
        t1.name = t2.name implies t1 = t2))
  end
\end{verbatim}
\normalsize

Another well-formedness rule requires that the starting state must
be one of the states of the state machine:

\small
\begin{verbatim}
context StateMachine::StateMachine
  @Constraint ValidStartingState
    not self.states->isEmpty implies self.states->includes(self.startingState)
  end
\end{verbatim}
\normalsize

The constraint language used in XMOF is OCL. The primary
difference between the OCL used here and the standard OCL language
is in the use of a different syntax for declarations. In this case
''@Constraint'' is used as opposed to the ''inv:'' declaration used
in standard OCL. The reasons for this choice will become apparent
later when we consider the need for a flexible parsing language.

\subsection{Queries}

OCL can be used to write queries. A query is used to produce a
value in the context of a current object state; it does not cause
any side effects. The following is an example of a query:

\small
\begin{verbatim}
@Class StateMachine
  @Operation getState(n:String):State
    self.states->select(s | s.name = n)->sel
  end
end
\end{verbatim}
\normalsize

This will filter the states of a state machine, selecting those
states whose name matches the string n. Here, sel, is an inbuilt
operation, which selects a single element from a collection. This
is required in order to return a single State. sAgain, note that
the declaration of a query diffes from that in the OCL standard.

\noindent Another example of query returns true if there exists a
state with the name, n:

\small
\begin{verbatim}
@Class StateMachine
  @Operation isState(n:String):Boolean
    self.states->exists(s | s.name = n)
  end
end
\end{verbatim}
\normalsize

\subsection{Actions and XOCL}

OCL is by design a static language and does not change the state of
objects it refers to.  In some situations this is a good thing
because it guarantees side-effect free evaluation.  However this
limitation makes it very difficiult to describe operational
behaviour in a way which can be readily executed.  Standard OCL
does provide pre-/post- conditions as a way of specifying the
effect of an operation, however, in general these cannot be
executed.

A more useful approach is to augment OCL with action primitives.
The XOCL language extends OCL with a number of key behaviour
primitives, as chapter \ref{} demonstrates, this is a essential
step towards making XMOF a true meta-programming environment.

An example of the application of actions in XOCL can be seen in
the state machine of figure \ref{classDiagram}. If it was
requirement to be able to add new states to the state machine
dynamically then the following XOCL statement can be written:

\small
\begin{verbatim}
context StateMachine
  @Operation addState(name:String)
    self.states := self.states->including(State(name))
  end
end
\end{verbatim}
\normalsize

New instances of classes can be created by declaring the class as
an operation. In this example a new instance of a State is created
by the declaration \emph{State()}. The resulting object is then
assigned to the set of states that includes the new state using the
assignment expression \emph{:=}. It is important to recognise that
\emph{:=} and \emph{new} have an imperative semantics and (given an
appropriate implementation) can be executed.

In the above example, the State() operation takes initialisation
value, which is the name of the state that is to be created. To
handle initialisation parameters, a special operation called init()
is provided. It takes a sequence of values as an argument, which
are then used to intialise the object's slots. In the case of the
state machine, three such operations are required, one for each
concrete class. The first intialises the name of a state, the
second assigns a name, and a source and target state to a
transition, and the third initialises a new state machine with a
starting state, set of transitions, and set of states:

\small
\begin{verbatim}
context State
  @Operation init(args)
    self.name := args->at(0)
  end
end

context Transition
  @Operation init(args)
     self.name := args->at(0);
     self.source := args->at(1);
     self.target := args->at(2)
  end

context StateMachine
  @Operation init(args)
     self.startingState := args->at(0);
     self.states := args->at(1);
     self.transitions := args->at(2)
  end
\end{verbatim}
\normalsize

The body of the next example illustrates how OCL conditional
expressions and logical operators can be combined with XOCL actions
to define the operation of adding a transition. This operation
takes the name the new transition and the name of a source and
target state. The isState() query is then used to check that the
states belong to the statemachine before creating a transition
between them. The last line of the if statement shows how XOCL
deals with the printing of strings to the terminal.

\small
\begin{verbatim}
context StateMachine
@Operation addTransition(name:String,source:String,target:String)
  let s = State(source);
      t = State(target) in
    if self.isState("source") and self.isState("target") then
      self.transitions := self.transitions->including(Transition(name,s,t))
    else
      "Invalid State in addTransition()".println()
    end
  end
end
\end{verbatim}
\normalsize

As this example show, augmenting OCL with a small number of action
primitives results in a powerful and expressive programming
language. Furthermore, as we will see in later chapters of this
book, because the language works at the XMOF level, it also
provides a rich meta-programming environment that can be used to
construct powerful modelling facilities such as model simulators,
execution engines and compilers. Indeed, it is sufficiently
expressive to enable a complete definition of all the languages in
this book to be constructed.

\subsection{Snapshots}

A useful notation for visually representing the instances of a
metamodel is a snapshot - a notation popularised by the Catalysis
method \cite{Catalysi}. A snapshot shows objects, the values of
their slots (instances of attributes) and links (instances of
associations). A snapshot of a metamodel will thus show objects and
links that are instances of elements in the metamodel. The example
shown in figure \ref{snapshotExample} is a snapshot of the
statemachibe metamodel, and shows an instance of a statemachine
containing three states and two transitions.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=8cm]{XMOF/figures/snapshot.pdf}
\caption{A snapshot showing an instance of the statemachine metamodel}
\label{snapshotExample}
\end{center}
\end{figure}

\subsection{Mappings}

Chapter \ref{} highlighted the fact that many languages are used
to design systems from a multitude of perspectives.  There must
exist relationships between the perspectives in order to understand
what one model means in terms of another.  These relationships are
implemented by a mapping language which specifies how we can
translate one language into another.  The mapping language used,
XMap, is a declarative, but executable language based on pattern
matching. Whilst this language can be viewed as a XMOF plug-in (as
opposed to a core part of the XMOF language), it is nevertheless
important for its ability express mappings in an intuitive, yet
ultimately implementable way.

To illustrate the use of XMap, figure \ref{cppExample} shows a
simple model of {C++} classes which will be used as the target of a
mapping from a state machine.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=8cm]{XMOF/figures/cppExample}
\caption{A simple model of C++ classes}
\label{cppExample}
\end{center}
\end{figure}

A {C++} class is a namespace for its attributes and operations
(methods). An attribute has a type, and for the purposes of this
example, its type may either be another class or an enumeration
type. An enumeration type has a value, which is the sequence of
strings in the enumeration. An operation has a name and a body,
which contains a simple string representation of the body of the
operation.

A mapping from from the state machine model in figure
\ref{classDiagram}  to the {C++} in \ref{cppExample} can be
defined. This maps a state machine to a {C++} class, where each
state in the state machine is mapped to a value in an enumerated
type called STATE. Eeach transition in the state machine is mapped
to a {C++} operation with the same name and a body, which changes
the state attribute to the target of the transition.

The mapping can be modelled in XMap as shown in figure
\ref{mapping}.  The arrows represent mappings between elements of
the two languages. The first mapping, SM2Class, maps a state
machine to a C++ class. The second mapping, Transition2Op, maps a
transition to an operation.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=8cm]{XMOF/figures/cppMapping}
\caption{A mapping between state machines and C++ classes}
\label{mapping}
\end{center}
\end{figure}

In order to describe the details of the mapping, XMap uses a
textual  mapping language based on pattern matching. Working
backwards, the definition of the mapping between a transition and
an operation is as follows:

\small
\begin{verbatim}
@Map Transition2Op
  @Clause Anonymous
    @Object(StateMachine::Transition,t)
      @Slot name = N end
    end
    when true
    do
    @Object(CPP::Operation)
      @Slot name = N end
      @Slot body = B end
    end
    where
      B = "state := " + self.target.name
  end
end
\end{verbatim}
\normalsize

A mapping consists of a collection of clauses, which are pattern
matches between source and target objects. Whenever a source object
is successfully matched to the input of the mapping, the resulting
object in the do expression is generated. Variables can be used
within clauses, and matched against values of slots in objects.
Because XMap builds on XOCL, XOCL expressions can also be used to
capture complex relationships between variables.

In this example, whenever the mapping is given a Transition with a
name equal to the variable N, it will generate an instance of the
class Operation, whose name is equal to N and whose body is equal
to the variable B. The where clause is used to define values of
variables, and it is used here to define the variable B to be
concatanation of the text "state := " with the target state name.
For instance, given a transition between the states "On" and "Off",
the resulting operation will have the body "state := Off". Note
that it would be quite possible to model a part of the syntax of
{C++} expressions, and equate B with an instance of an expression.

The mapping between state machines and {C++} classes is shown below:

\small
\begin{verbatim}
 @Map SM2Class
   @Clause Anonymous
     @Object(StateMachine::StateMachine)
       @Slot states = S end
       @Slot transitions = TS end
     end
     when true
     do
     @Object(CPP::CPPClass)
       @Slot attributes =
         Set{@Object(CPP::CPPAtt)
           @Slot name = "state" end
           @Slot type = T end
         end}
       end
       @Slot operations = O end
     end
     where
       T = @Object(CPP::EnumerationType)
         @Slot name = "STATE" end
         @Slot value = S->iterate(s Q=Seq{} | Q + s.name)
       end
       end;
       O = TS->collect(t | (Transition2Op.new())(t))
    end
  end
end
\end{verbatim}
\normalsize

Here, a state machine with a set of states, S, and a set of
transitions, TS, is mapped to a {C++} class with a distinguised
attribute "state" of type T, and a set of operations, O. The value
of T is an EnumerationType whose name is "STATE" and whose values
are the names of the states in S. Finally, the transitions are
mapped to operations by iterating through the transitions in TS and
applying the Transition2Op mapping.

This mapping illustrates the power of the XMap language in being
able to match arbritrarily complex structures of source and target
objects. For example, as shown by the CPPClass, source and target
objects may be nested within objects to any depth, whilst complex
rules for determining the values of slots in objects can be readily
constructed in OCL.

\subsection{Concrete Syntax}

The concrete syntax of a modelling language defines the notation
that is used to present models in the language. A notation may be
textual, or diagrammatical, or a mxuture of both. A key part of any
metamodelling language is the ability to model both these aspects,
and as a result facilitate the rapid creation of parsers and
diagram editors for a new language.

\subsection{Textual Syntax}

XMOF provides a generic parser language that can be used to model
the textual syntax of any language. This language, called XBNF (the
reader will be starting to see a pattern to our naming conventions
by now!) allows new textual constructs to be defined that can be
used as input to a model parser.

\noindent These new constructs to be defined as:

\small
\begin{verbatim}
@<NAME>
  <BODY>
end
\end{verbatim}
\normalsize

\noindent where <NAME> is the name of the construct and <BODY> is
an XBNF expression.

An XBNF expression consists of a number of BNF definition within
which XOCL variables are embedded, followed by an XOCL expression.
When a construct is parsed, the XBNF expression is used to match
each parsed element with the variables. These variables can then be
used within the XOCL action to create instances of classes that
populate a language metamodel.

Imagine that we wish to create a concrete syntax for the simple
state machine example. One part of this task would be to create a
concrete syntax for states. This might take the form:

\small
\begin{verbatim}
@State On
end
@State Off
end
\end{verbatim}
\normalsize

The following XBNF defines the syntax for parsing states and
populating instances of the class State.

\small
\begin{verbatim}
State ::= 'state' '(' name = Name ')' {State(name)}
\end{verbatim}
\normalsize

\noindent Now we have a new construct. When we type:

\small
\begin{verbatim}
  @State X end
\end{verbatim}
\normalsize

\noindent we will get:

\small
\begin{verbatim}
<State X> returned.
\end{verbatim}
\normalsize

\section{XMOF Metamodel}

As outlined in the previous chapter, XMOF follows the golden braid
metamodel architecture, and therefore is metamodelled in its own
language. Understanding the architecture of this metamodel is
important for many reasons. Firstly, the architecture is a good
example of an XMOF metamodel definition in its own right - the fact
that the XMOF metamodel is both self describing and self supporting
makes a strong statement about the expressibility of the language.
Secondly, the XMOF metamodel acts as a root for many other
metamodel definitions. For instance, it can be viewed as a subset
of the UML metamodel, and many other types of modelling languages
can also be viewed as extensions of the core architecture.

Figure \ref{xmofOverview} shows the key components of the XMOF
metamodel. The classes and relationships in the metamodel
correspond precisely to the modelling features that have been used
in this chapter to model the abstract syntax, semantics and
concrete syntax of the statemachine language. For example, the
package and classes shown in the state machine abstract syntax
metamodel in figure \ref{classDiagram} can be viewed as concrete
syntax representations of instances of the classes XMOF::Package
and XMOF::Package. The concrete syntax model can be viewed as a
representation of an instance of the class Grammar, and so on.

\begin{figure}[htb]
\begin{center}
\includegraphics[height=17cm]{XMOF/figures/XMOFSimple.pdf}
\caption{Overview of XMOF Architecture}
\label{xmofOverview}
\end{center}
\end{figure}

As we discuss the modelling of abstract syntax and semantics in
more detail in later chapters, many of the features of the
metamodel will become more understandable. There are however, some
key features that it is useful to point out here.

\begin{description}
\item[Elements and Objects] The most fundemental modelling concepts in XMOF are
elements and objects. Elements are the root of all modelling concepts, in other
words, every type of modelling concept in XMOF is an element. Elements do not
have structure or state. Objects on the hand are elements that encapsulate data
values - called slots in XMOF. An object's slots must conform to the name and
type of the attributes of the class it is an instance of.
\item[Performable] The performable class represents the root of all modellng
concepts that can be evaluated in the context of an environment (a collection
of variable bindings) to return a result. An OCL expression is a good example
of a performable concept.
\item[Classification] In XMOF, some types of modelling elements
are modelled as Classifiers. A Classifier is an element that can be
instantiated via the new() operation to create new instances. Good
examples of these elements are classes and datatypes, which can be
instantiated to create objects and datavalues. All elements have an
of() operation, which returns the classifier that the element was
instantiated from. So for example, the objects statemachine1, statemachine2
will return the class StateMachine, whilst the object fido, might return
the class Dog.
\item[Reflection]
An important property of all XMOF models is that classifiers are also objects.
This apparently strange assumption means that effectively classes and datatypes
can also be viewed as being instances of classifiers. In this case, they will
be instances of the classes XMOF::Class and XMOF::DataType. This capability
is an important one, as it enables any operation that can be carried out on
an object such as executing its operations, or mapping it to another object
can also be applied to elements at the XMOF level.
\item[XOCL] The XOCL class is an extension of OCL, and is the root of all
imperative expressions that can change the state of a model (not shown here).
\item[Snapshot] A snapshot is a collection of elements, and may therefore
include any type of element that is availble in XMOF.
\item[Grammar] A grammar can be evaluated in the context of sequence of
tokens to generate an instance of a model.
\end{description}

\section{Extensions to support reuse}

Metamodels can often be complex and time consuming to construct.
Because  the metamodelling languages is OO then some support for
reuse of metamodels is provided using class specialisation.  The
problem with this type of reuse in the context of metamodels is
that it is too fine grained.  Metamodels often share architectural
patterns, the components of which are distributed across many
classes.  It is these architectural patterns that need to be reused
rather than their components.  One solution to this is a coarse
grained reuse mechanism called templates which is also included in
UML 2.0.  Templates enable patterns to be encapsulated into
reusable units that can subsequently be used to define metamodels.
XMOF utilises templates as one of its key reuse mechanisms.

Figure \ref{templateExample} shows an example of the application to
templates to the class diagram of figure \ref{classDiagram}.  In
this the \emph{Namespace} template describes a pattern where a
\emph{Namespace} owns a number of \emph{NamedElement}.  The OCL
constraint augments this definition by specifying that each of the
named elements must have a distinct name.  A concrete metamodel is
derived from templates by passing parameters into one or more
templates.  In the case of figure \ref{templateExample},
\emph{Namespace} is substituted for \emph{StateMachine} and
\emph{NamedElement} for \emph{State} in one instantiation of the
template, and \emph{Namespace} is substituted for
\emph{StateMachine} and \emph{NamedElement} for \emph{Transition}
in a further instantiation.  The resulting definition is merged,
but more details of that will be given in chapter \ref{}.  The
important point is that the resulting metamodel is
indistinguishable from the one shown in figure \ref{classDiagram}.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=10cm]{XMOF/figures/templateExample}
\caption{Using a template to derive the class diagram of figure \ref{classDiagram}}
\label{templateExample}
\end{center}
\end{figure}

\section{Differences from Existing Metamodelling Languages}

The requirement to be able to construct metamodels is not a new
one, and not surprisingly a variety of languages have been proposed
as metamodelling languages. The most notable of these are UML and
the MOF (the Meta Object Fa cility). The MOF is the standard
language for capturing meta-data, and goes further than the UML in
meeting the requirements of a metamodelling language. Nevertheless,
whilst the MOF provides many of the features necessary to define
metamodels, there are a number of crucial areas in which it needs
to be extended.

\begin{itemize}
\item The MOF does not explicitly support executable metamodelling in
a platform independent way. Although it does provide OCL, this does not
support the construction of operations that change the state of a model.
An alterantive might be to use the Action semantics. This is a platform
independent language for executing models, that is currently a part of
the the UML 1.5 metamodel. There are two main problems with this language
however. It is complex and does not support many of the useful set
operations offered by OCL, such as iterate, collect and select. Secondly,
it is not currently a part of the MOF metamodel. Whilst work is ongoing
 to resolve these issues, XMOF resolves them by the minimal extension of
 OCL to result in the powerful executable expression language.
\item The MOF does not support an extensible grammar language. This is
important in being able to model new concrete syntax grammars in MOF.
\item The MOF currently is not defined fully in terms of itself. Its
semantics and syntax are stated in a form (a mixture of OCL, and
informal english) that prevents it from being completely self describing
and self supporting.
\item The MOF currently does not support a pattern based mapping language
such as the XMap language described above. Work is howwever, currently
proceeding on an extension to MOF called QVT (Queries, Views, Transformations),
which aims to define a language for doing mappings, but it is unlear at this
stage whether it will support all the capabilities of XMap in the short to
medium term.
\end{itemize}

XMOF aims to provide these extensions in the most concise and
minimal fashion necessary to support precise, semantically rich
metamodelling.


\section{Conclusions}


==> XMF/xmof.tex <==
\chapter{A Language for Metamodelling}
\label{xmofchapter}

\section{Introduction}

In order to be able to construct models of languages, a modelling
language is required. This language is known as a {\em
metamodelling language}. A metamodelling language should provide
the ability to capture the key features of a modelling language,
including its syntax and semantics in a unified and platform
independent way. This chapter introduces an object-oriented
metamodelling language called XMOF (eXecutable MOF) that does just
this. XMOF is an extension to existing standards for metamodelling
such as MOF, OCL and QVT that is rich enough to address all the
requirements of metamodelling. This will form the foundation for
exploring metamodelling throughout the rest of this book.

\section{Requirements of a Metamodelling Language}

Before introducing XMOF, it is important to understand some of the
key requirements of a metamodelling language.

Firstly, as described in the previous chapter, a metamodel should
capture all the essential features of a modelling language. Thus,
a metamodelling language should provide modelling concepts that
can capture the abstract syntax, concrete syntax and semantics of
a language. In addition, it should provide facilities for
manipulating metamodels, including the ability to map them to
other metamodels and extend metamodels to support new language
definitions.

Secondly, a metamodelling language should itself be completely
described by its metamodel, thus ensuring that the language is
self defined and complete, and enabling its definition to be
rapidly reused to create new language metamodels.

Finally, to gain maximum flexibility, a metamodelling language
must be platform independent. In other words, the resulting
metamodels should be self sufficient and independent of
implementation specific descriptions of the language being
modelled. Thus, reliance on the implementation of the language's
behaviour in an external programming language or the assumption
that there will be an external database that manages object
creation and persistence is completely avoided.

\subsection{XMOF}

The metamodelling language presented in this chapter aims to
provide a rich environment for language design that supports the
key requirements of a metamodelling language. This language,
called XMOF, combines and extends a number of standard
object-oriented modelling facilities to provide a minimal, but
expressive, platform independent language for metamodelling. XMOF
includes the following features:

\begin{itemize}

\item Support for standard OO modelling concepts such as packages, classes, and
associations to describe language concepts and their relationship to one another.

\item A constraint language, which can used to describe well-formedness rules.

\item A set of action primitives, which can be used to capture the behavioural
semantics of a language. This turns XMOF into a meta-programming
language.

\item A language for expressing mappings (both uni-directional and bi-directional)
between languages and language components.

\item A concrete syntax language which can be used to model the concrete syntax of
any modelling language.

\item A generic metamodel framework, which supports standard plug-points and machinery for
expressing model element instantiation, execution, expression evaluation and reflection.

\item Conformance to the golden-braid metamodel architecture
described in section \ref{goldenbraid}, ensuring that the
language, including its semantics is completely self describing.

\end{itemize}

The following sections present an overview of the key features of
XMOF. This is not a full definition, but will reference fuller
descriptions of the components of the language where appropriate.

\section{XMOF Features}

\subsection{OO modelling concepts}

XMOF provides the standard OO modelling concepts that are
supported by MOF and UML, including packages, classes and
associations. These are  visualised using class diagrams. Figure
\ref{classDiagram} shows an example of a class diagram of a simple
model consisting of a package with a number of classes and
associations. This model describes a simple StateMachine, where a
StateMachine contains States and Transitions, and Transitions have
source and target states.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=11cm]{XMOF/figures/classDiagramExample}
\caption{An example of a class diagram}
\label{classDiagram}
\end{center}
\end{figure}

XMOF also provides a concrete syntax for packages and classes. The
equivalent concrete representation of the StateMachine class
diagram shown in figure \ref{classDiagram} is shown below.

\small
\begin{verbatim}
1 @Package StateMachines
2    @Class isAbstract Named
3      @Attribute name : String end
4    end
5    @Class StateMachine extends Named
6      @Attribute states : Set(State) end
7      @Attribute transitions : Set(Transition) end
8      @Attribute startingState : State end
9    end
10   @Class State extends Named
11   end
12   @Class Transition extends Named
13     @Attribute source : State end
14     @Attribute target : State end
15   end
16 end
\end{verbatim}

\normalsize

Here, line 1 shows the start of a package named StateMachine,
which contains all the sub-definitions relating to StateMachines.

Line 2 contains the start of a class definition for the class
Named,  which is an abstract class for a named element. Line 5 is
the start of the definition of the StateMachine class. It defines
two attributes named states and transitions, whose types are
Set(State) and Set(Transition). These types correspond to the "*"
multiplicity of the equivalent association ends in the class
diagram.

Lines 10 and 12 are the start of the State and Transition class
definitions. Both these classes specialise the class Named, and
therefore inherit a name attribute. A Transition has two attributes
source and target, which are of type State. The fact that they are
single valued reflects the multiplicity of the equivalent
association ends in the class diagram.

As chapter \ref{concretechapter} will show, the concrete
representation of a modelling language should be clearly
distinguished from its abstract syntax representation. Here, two
different concrete syntaxes are being used to capture the same
information.

\subsection{Imports}

Just as in UML and MOF, a package can be imported into another
package using import. The result is that all referenceable
elements in the imported package can be referenced by elements in
the importing package. Consider the following package:

\small
\begin{verbatim}
@Package X
  @Class Y end
end

@Package A imports X
  @Class B
    @Attribute b : Y end
  end
end
\end{verbatim}
\normalsize

Because the package A imports the package X, then elements in the
package X can be referenced without the need to provide a full
path name.

In addition, XMOF packages can import parsers. Once a parser has
been imported, the syntax and semantics of the language it
supports is immediately available. Thus, the developer can pick
and mix languages that best fit the problem domain. This
capability is an essential part of the flexibility offered by
XMOF's meta-programming environment.

\subsection{Constraints}

It is often necessary to make well-formedness statements about
concepts in a model.  These statements are often made informally,
for example in the context of figure \ref{classDiagram} it might
be useful to specify that \emph{all transitions have unique names
within a state machine}. A constraint language provides a means of
succinctly and unambiguously expressing complex well-formedness
rules. For example the well-formedness statement mentioned above
can be added to the class StateMachine in the following way:

\small
\begin{verbatim}
context StateMachines::StateMachine
  @Constraint NoTwoTransitionsWithTheSameName
    self.transitions->forAll(t1 |
      self.transition->forAll(t2 |
        t1.name = t2.name implies t1 = t2))
  end
\end{verbatim}
\normalsize

Another well-formedness rule requires that the starting state must
be one of the states of the state machine:

\small
\begin{verbatim}
context StateMachines::StateMachine
  @Constraint ValidStartingState
    not self.states->isEmpty implies
      self.states->includes(self.startingState)
  end
\end{verbatim}
\normalsize

The constraint language used in XMOF is OCL \cite{Warmer}. The
primary difference between the OCL used here and the standard OCL
language is in the use of a different syntax for declarations. In
this case ''@Constraint'' is used as opposed to the ''inv:''
declaration used in standard OCL. The reasons for this choice will
become apparent later when we consider the need for a flexible
parsing language.

\subsection{Queries}

OCL can be used to write queries. A query is used to produce a
value in the context of a current object state; it does not cause
any side effects. The following is an example of a query:

\small
\begin{verbatim}
@Class StateMachines
  @Operation getState(n:String):State
    self.states->select(s | s.name = n)->sel
  end
end
\end{verbatim}
\normalsize

This will filter the states of a state machine, selecting those
states whose name matches the string n. Here, sel, is an in-built
operation, which selects a single element from a collection. This
is required in order to return a single State. Again, note that
the declaration of a query differs from that in the OCL standard.

\noindent Another example of query returns true if there exists a
state with the name, n:

\small
\begin{verbatim}
@Class StateMachines
  @Operation isState(n:String):Boolean
    self.states->exists(s | s.name = n)
  end
end
\end{verbatim}
\normalsize

\subsection{Actions and XOCL}

OCL is by design a static language and does not change the state
of objects it refers to.  In some situations this is a good thing
because it guarantees side-effect free evaluation.  However this
limitation makes it very difficult to describe operational
behaviour in a way which can be readily executed.  Standard OCL
does provide pre-/post- conditions as a way of specifying the
effect of an operation, however in general these cannot be
executed.

A better approach is to augment OCL with action primitives. The
XOCL (eXecutable OCL) language extends OCL with a number of key
behaviour primitives. This is a essential step towards making XMOF
a true meta-programming environment.

An example of the application of actions in XOCL can be seen in
the state machine of figure \ref{classDiagram}. If it was required
to add new states to the state machine dynamically then the
following XOCL statement can be written:

\small
\begin{verbatim}
context StateMachines
  @Operation addState(name:String)
    self.states := self.states->including(State(name))
  end
end
\end{verbatim}
\normalsize

New instances of classes can be created by declaring the class as
an operation. In this example a new instance of a State is created
by the declaration State(). The resulting object is then assigned
to the set of states that includes the new state using the
assignment expression \emph{:=}. It is important to recognise that
\emph{:=} and \emph{new} have an imperative semantics and (given
an appropriate implementation) can be executed.

In the above example, the State() operation takes an
initialisation value, which is the name of the state that is to be
created. To handle initialisation parameters, a special operation
called a constructor is provided. It takes a sequence of values as
an argument, which are then used to intialise the object's slots.
In the case of the state machine, three contructors are required,
one for each concrete class. The first intialises the name of a
state, the second assigns a name, and a source and target state to
a transition, and the third initialises a new state machine with a
starting state, set of transitions, and set of states. Note, that
if the body of the constructor is empty, the default action is to
set the attribute values (slots) of the created object with the
values of the parameters.

\small
\begin{verbatim}
context State
  @Constructor(name)
  end

context Transition
  @Constructor(name,source,target)
  end

context StateMachine
  @Constructor(name,source,target)
  end
\end{verbatim}
\normalsize

The body of the next example illustrates how OCL conditional
expressions and logical operators can be combined with XOCL
actions to define the operation of adding a transition. This
operation takes the name of the new transition and the name of a
source and target state. The isState() query is then used to check
that the states belong to the StateMachine before creating a
transition between them. The last line of the if statement shows
how XOCL deals with the printing of strings to the terminal.

\small
\begin{verbatim}
context StateMachines @Operation
addTransition(name:String,source:String,target:String)
  if self.isState(source) and self.isState(target) then
    self.transitions := self.transitions->
      including(Transition(name,s,t))
  else
    "Invalid State in addTransition()".println()
  end
end
\end{verbatim}
\normalsize

As this example show, augmenting OCL with a small number of action
primitives results in a powerful and expressive programming
language. Furthermore, as we will see in later chapters of this
book, because the language works at the XMOF level, it also
provides a rich meta-programming environment that can be used to
construct powerful modelling facilities such as model simulators,
execution engines and compilers. Indeed, it is sufficiently
expressive to enable a complete definition of all the languages in
this book to be constructed.

\subsection{Snapshots}

A useful notation for visually representing the instances of a
metamodel is a snapshot - a notation popularised by the Catalysis
method \cite{Catalysis}. A snapshot shows objects, the values of
their slots (instances of attributes) and links (instances of
associations). A snapshot of a metamodel will thus show objects
and links that are instances of elements in the metamodel. The
example shown in figure \ref{snapshotExample} is a snapshot of the
StateMachine metamodel, and shows an instance of a StateMachine
containing three states and two transitions.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=11cm]{XMOF/figures/snapshot.pdf}
\caption{A snapshot showing an instance of the statemachine metamodel}
\label{snapshotExample}
\end{center}
\end{figure}

\subsection{Mappings}

Chapter \ref{mddchapter} highlighted the fact that many languages
are used to design systems from a multitude of perspectives. There
must exist relationships between the perspectives in order to
understand what one model means in terms of another.  These
relationships are implemented by a mapping language which
specifies how we can translate one language into another.  The
mapping language used, XMap, is a declarative, executable language
based on pattern matching. Whilst this language can be viewed as a
XMOF plug-in (as opposed to a core part of the XMOF language), it
is nevertheless important for its ability express mappings in an
intuitive, yet ultimately implementable way.

To illustrate the use of XMap, figure \ref{cppExample} shows a
simple model of {C++} classes which will be used as the target of a
mapping from a state machine.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=11cm]{XMOF/figures/cppExample}
\caption{A simple model of C++ classes}
\label{cppExample}
\end{center}
\end{figure}

A {C++} class is a namespace for its attributes and operations
(methods). An attribute has a type, and for the purposes of this
example, its type may either be another class or an enumeration
type. An enumeration type has a value, which is the sequence of
strings in the enumeration. An operation has a name and a body,
which contains a simple string representation of the body of the
operation.

A mapping from from the StateMachine model in figure
\ref{classDiagram} to the {C++} in \ref{cppExample} can be
defined. This maps a StateMachine to a {C++} class, where each
state in the state machine is mapped to a value in an enumerated
type called STATE. Each transition in the state machine is mapped
to a {C++} operation with the same name and a body, which changes
the state attribute to the target of the transition.

The mapping can be modelled in XMap as shown in figure
\ref{mapping}.  The arrows represent mappings between elements of
the two languages. The first mapping, SM2Class, maps a state
machine to a C++ class. The second mapping, Transition2Op, maps a
transition to an operation.

\begin{figure}[htb]
\begin{center}
\includegraphics[width=11cm]{XMOF/figures/cppMapping}
\caption{A mapping between state machines and C++ classes}
\label{mapping}
\end{center}
\end{figure}

In order to describe the details of the mapping, XMap uses a
textual  mapping language based on pattern matching. Working
backwards, the definition of the mapping between a transition and
an operation is as follows:

\small
\begin{verbatim}
@Map Transition2Op
  @Clause Transition2Op
    Transition
      [name = N,
       target = T]
    when true
    do
    Operation
      [name = N,
       body = B]
    where
      B = "state = " + T.name
  end
end
\end{verbatim}
\normalsize

A mapping consists of a collection of clauses, which are pattern
matches between source and target objects. Whenever a source object
is successfully matched to the input of the mapping, the resulting
object in the do expression is generated. Variables can be used
within clauses, and matched against values of slots in objects.
Because XMap builds on XOCL, XOCL expressions can also be used to
capture complex relationships between variables.

In this example, whenever the mapping is given a Transition with a
name equal to the variable N and a target equal to T, it will
generate an instance of the class Operation, whose name is equal
to N and whose body is equal to the variable B. The where clause
is used to define values of variables, and it is used here to
define the variable B to be concatenation of the text "state := "
with the target state name. For instance, given a transition
between the states "On" and "Off", the resulting operation will
have the body "state := Off". Note that it would be quite possible
to model a part of the syntax of {C++} expressions, and equate B
with an instance of an expression.

The mapping between state machines and {C++} classes is shown below:

\small
\begin{verbatim}
 @Map SM2Class
   @Clause SM2Class
     StateMachine
       [states = S,
        transitions = TS]
     when true
     do
     CPPClass
       [attributes =
         Set{CPPAtt
           [name = "state",
            type = T]},
        operations = O]
     end
     where
       T = EnumerationType
         [name = "STATE",
          value = S->iterate(s Q=Seq{} | Q + s.name)];
       O = TS->collect(t | Transition2Op()(t))
    end
  end
end
\end{verbatim}
\normalsize

Here, a state machine with a set of states, S, and a set of
transitions, TS, is mapped to a {C++} class with a distinguised
attribute state of type T, and a set of operations, O. The value
of T is an EnumerationType whose name is ``STATE'' and whose
values are the names of the states in S. Finally, the transitions
are mapped to operations by iterating through the transitions in
TS and applying the Transition2Op mapping.

This mapping illustrates the power of the XMap language in being
able to match arbitrarily complex structures of source and target
objects. For example, as shown by the CPPClass, source and target
objects may be nested within objects to any depth, whilst complex
rules for determining the values of slots in objects can be
readily constructed in OCL.

\subsection{Synchronised Mappings}

Whilst it is common to want to translate from one language to
another, there is also a requirement to keep different models in
step. For example, an abstract syntax model may need to be kept in
step with a model of its concrete syntax, or a business model may
need to be synchronised with code. To achieve this, XMOF provides
a bi-directional mapping language. This enables rules to be
defined that state how models at either end of a mapping must
change in response to changes at the other end, thus providing a
declarative language for synchronisation. This language will be
explored in greater detail in chapter \ref{mappingchapter}.

\subsection{Concrete Syntax}

The concrete syntax of a modelling language defines the notation
that is used to present models in the language. A notation may be
textual, or diagrammatical, or a mixture of both. A key part of
any metamodelling language is the ability to model both these
aspects in a platform independent way, and as a result facilitate
the rapid creation of parsers and diagram editors for a new
language.

\subsection{Textual Syntax}

XMOF provides a generic parser language that can be used to model
the textual syntax of any language. This language, called XBNF
(the reader will be starting to see a pattern to our naming
conventions by now!) allows new textual constructs to be defined
that can be used as input to a model parser. These new constructs
to be defined as:

\small
\begin{verbatim}
@<NAME>
  <BODY>
end
\end{verbatim}
\normalsize

\noindent where {\tt <NAME>} is the name of the construct and{\tt
<BODY>} is an XBNF expression.

An XBNF expression consists of a number of EBNF definitions within
which XOCL variables are embedded, followed by an XOCL expression.
When a construct is parsed, the XBNF expression is used to match
each parsed element with the variables. These variables can then
be used within the XOCL action to create instances of classes that
populate a model of the abstract syntax of a language.

Imagine that we wish to create a concrete syntax for the simple
StateMachine example. One part of this task would be to create a
concrete syntax for states. This might take the form:

\small
\begin{verbatim}
@State On
end
@State Off
end
\end{verbatim}
\normalsize

The following XBNF defines the syntax for parsing states and
populating instances of the class State.

\small
\begin{verbatim}
State ::= name = Name {[| State(name) |]}
\end{verbatim}
\normalsize

\noindent Now we have a new construct. When we type:

\small
\begin{verbatim}
  @State X end
\end{verbatim}
\normalsize

\noindent we will get:

\small
\begin{verbatim}
<State X> returned.
\end{verbatim}
\normalsize

\subsection{Diagrammatical Syntax}

In order to model the diagrammatical syntax of a modelling
language, XMOF provides a generic model of diagram elements such
as boxes, lines, etc, that can be tailored to support specific
types of diagrams. Bi-directional mappings are used to model the
relationship between a specific diagram model and the model of the
language's abstract syntax. This ensures that whenever changes are
made to a diagram, they are reflected in the model and vice versa.
By providing an interpreter (written in XMOF) for displaying
instances of a diagrammatical syntax model, it is possible to
construct new diagram editors for a specific modelling language in
very short timescales.

\section{XMOF Architecture}

As outlined in the previous chapter, XMOF follows the golden braid
metamodel architecture, and therefore is metamodelled in its own
language. Understanding the architecture of XMOF is important for
many reasons. Firstly, it provides a good example of a language
definition in its own right - the fact that XMOF is self
describing makes a strong statement about the expressibility of
the language. Secondly, XMOF acts as a root for many other
metamodel definitions. For instance, it can be viewed as a subset
of the UML metamodel, and many other types of modelling languages
can also be viewed as extensions of the core architecture.

Figure \ref{xmofOverview} shows the key components of the XMOF
architecture. At the heart of XMOF is a core or essential MOF
language metamodel. Around it sit the metamodels for the OCL,
XOCL, XBNF and XMap languages.

The classes and relationships in the metamodel correspond
precisely to the modelling features that have been used in this
chapter to model the abstract syntax, semantics and concrete
syntax of the StateMachine language. For example, the package and
classes shown in the StateMachine abstract syntax model in figure
\ref{classDiagram} can be viewed as concrete syntax
representations of instances of the classes Core::Package and
Core::Class. The concrete syntax model can be viewed as a
representation of an instance of XBNF::Grammar, and so on.

\begin{figure}[htb]
\begin{center}
\includegraphics[height=10cm]{XMOF/figures/XMOFOverview.pdf}
\caption{Overview of XMOF Architecture} \label{xmofOverview}
\end{center}
\end{figure}

\subsection{Core Metamodel}

As shown in figure \ref{coreMetamodel}, the classes that are
defined in the core metamodel provide the core concepts used in
XMOF such as Class and Package. As we discuss metamodelling in
more detail in later chapters, many of the features of the
metamodel will become more understandable.

\begin{figure}[htb]
\begin{center}
\includegraphics[height=17cm]{XMOF/figures/XMOFSimple.pdf}
\caption{Core or Essential XMOF Metamodel} \label{coreMetamodel}
\end{center}
\end{figure}

\noindent There are however, some key features that it is useful
to point out here:

\begin{description}
\item[Elements and Objects] The most fundamental modelling concepts in XMOF are
elements and objects. Elements are the root of all modelling
concepts, in other words, every type of modelling concept in XMOF
is an element. Elements do not have structure or state. Objects on
the other hand are elements that encapsulate data values - called
slots in XMOF. An object's slots must conform to the name and type
of the attributes of the class it is an instance of.
\item[Performable] The performable class represents the root of all modellng
concepts that can be evaluated in the context of an environment (a collection
of variable bindings) to return a result. An OCL expression is a good example
of a performable concept.
\item[Classification] In XMOF, some types of modelling elements
are modelled as Classifiers. A Classifier is an element that can
be instantiated via the new() operation to create new instances.
Good examples of these elements are classes and datatypes, which
can be instantiated to create objects and datavalues. All elements
have an of() operation, which returns the classifier that the
element was instantiated from. So for example, the objects
statemachine1, statemachine2 will return the class StateMachine,
whilst the object fido might return the class Dog.
\item[Reflection]
An important property of all XMOF models is that classes are also
objects. This apparently strange assumption means that classes and
datatypes can also be viewed as instances of classifiers. In this
case, they will be instances of the classes XMOF::Class and
XMOF::DataType. This capability is an important one, as it enables
any operation that can be carried out on an object such as
executing its operations, or mapping it to another object can also
be applied to elements at the XMOF level.
\item[XOCL] The XOCL class is an extension of OCL, and is the root of all
imperative expressions that can change the state of a model (not shown here).
\item[Snapshot] A snapshot is a collection of elements, and may therefore
include any type of element that is available in XMOF.
\item[Grammar] A grammar can be evaluated in the context of sequence of
tokens to generate an instance of a model.
\end{description}

\section{Relationship to Existing Metamodelling Languages}
\label{differences}

The requirement to be able to construct metamodels is not a new
one, and not surprisingly a variety of languages have been
proposed as metamodelling languages. The most notable of these are
UML and the MOF (the Meta Object Facility). The MOF is the
standard language for capturing meta-data, and goes further than
the UML in meeting the requirements of a metamodelling language.
Nevertheless, whilst the MOF provides many of the features
necessary to define metamodels, there are a number of crucial
areas in which it needs to be extended.

\begin{itemize}
\item The MOF does not explicitly support executable metamodelling in
a platform independent way. Although it does provide OCL, this
does not support the construction of operations that change the
state of a model. An alternative might be to use the Action
semantics. This is a platform independent language for executing
models, that is currently a part of the the UML 1.5 metamodel.
There are two main problems with this language however. It is
complex and does not support many of the useful set operations
offered by OCL, such as iterate, collect and select. Secondly, it
is not currently a part of the MOF metamodel. Whilst work is
ongoing to resolve these issues, XMOF resolves them by the minimal
extension of OCL, resulting in a powerful executable modelling
language.
\item The MOF does not support an extensible grammar language. This is
important in being able to model new concrete syntax grammars in MOF.
\item The MOF currently is not defined fully in terms of itself. Its
semantics and syntax are stated in a form (a mixture of OCL, and
informal English) that prevents it from being completely self
describing and self supporting.
\item The MOF currently does not support a pattern based mapping language
such as the XMap language described above. Work is currently
proceeding on an extension to MOF called QVT (Queries, Views,
Transformations), which aims to define a language for doing
mappings, but it is unclear at this stage whether it will support
all the capabilities of XMap in the short to medium term.
\end{itemize}

XMOF aims to provide these extensions in the most concise and
minimal fashion necessary to support precise, semantically rich
metamodelling.

\section{Conclusion}

This chapter has described some of the essential features of XMOF,
an extended MOF like language that provides the facilities
necessary to define complete, semantically rich metamodels of
languages. These facilities will be used throughout the rest of
this book to illustrate the metamodelling process in greater
detail.

